Convergence and Alignment of Gradient Descent with Random Backpropagation Weights

Stochastic gradient descent with backpropagation is the workhorse of artificial neural networks. It has long been recognized that backpropagation fails to be a biologically plausible algorithm. Fundamentally, it is a non-local procedure -- updating one neuron's synaptic weights requires knowledge of synaptic weights or receptive fields of downstream neurons. This limits the use of artificial neural networks as a tool for understanding the biological principles of information processing in the brain. Lillicrap et al. (2016) propose a more biologically plausible "feedback alignment" algorithm that uses random and fixed backpropagation weights, and show promising simulations. In this paper we study the mathematical properties of the feedback alignment procedure by analyzing convergence and alignment for two-layer networks under squared error loss. In the overparameterized setting, we prove that the error converges to zero exponentially fast, and also that regularization is necessary in order for the parameters to become aligned with the random backpropagation weights. Simulations are given that are consistent with this analysis and suggest further generalizations. These results contribute to our understanding of how biologically plausible algorithms might carry out weight learning in a manner different from Hebbian learning, with performance that is comparable with the full non-local backpropagation algorithm.

==> background.tex <==
%!TEX root=./main.tex
\section{Preliminaries}

In this paper, we consider a two-layer neural network $f:\Rd \to \RR$ with hidden-layer width $p$. For any input $x\in\Rd$, the network outputs
\begin{align}\label{eqn:nonlinear-network}
    f(x) = \frac{1}{\sqrt p}\sum_{r=1}^p\beta_r\psi(w_r\transpose x)= \frac{1}{\sqrt p}\beta\transpose\psi(Wx),
\end{align}
where $W = (w_1,...,w_p)\transpose\in\Rpd$ and $\beta = (\beta_1,...,\beta_p)\transpose\in\Rp$ represent the feed-forward weights for the first and the second layer, and $\psi$ denotes an element-wise activation function.
Given $n$ input-label pairs $\{(x_i,y_i)\}_{i=1}^n$, we hope to minimize the squared error loss
\begin{equation}\label{eqn:squared-loss}
    \Loss(W,\beta) = \frac{1}{2}\sum_{i=1}^n \big(f(x_i)-y_i\big)^2.
\end{equation}
Vanilla gradient descent minimizes \eqref{eqn:nonlinear-network} through updating the feed-forward weights following gradient directions, \ie,
\begin{align*}
    \beta_r(t+1) = \beta_r(t)-\eta\frac{\partial\Loss}{\partial \beta_r}(W(t),\beta(t)), \quad w_r(t+1) = w_r(t)-\eta\frac{\partial\Loss}{\partial w_r}(W(t),\beta(t)),
\end{align*}
where $\eta>0$ denotes the step size. In this paper, we initialize $\beta(0)$ and $w_r(0)$ for all $r\in[p]$ with standard Gaussian vectors. To simplify the notation, we introduce in the rest of this paper $u(t),e(t)\in \R^n$, where $u_i(t)$ denotes the network output on input $x_i$ at step $t$ and $e_i(t) = u_i(t)-y$ represents the corresponding prediction error.

\paragraph{Backpropagation on two-layer network.}

Backpropagation has been the most commonly used scheme for calculating the gradient of network parameters. In particular, for two-layer network \eqref{eqn:nonlinear-network}, the gradients with respect to the first- and second-layer weights under backpropagation write
\begin{equation*}
    \frac{\partial\Loss}{\partial \beta_r} = \frac{1}{\sqrt p}\sum_{i=1}^n e_i\psi(w_r\transpose x_i), \quad
    \frac{\partial\Loss}{\partial w_r} = \frac{1}{\sqrt p} \sum_{i=1}^n e_i \beta_r\psi'(w_r\transpose x_i)x_i.
\end{equation*}
However, such learning algorithm requires updating its weights with backpropagated error signals that consist of non-local information of weight parameters from top layers. More specifically, given an input $x_i$, the gradient of second-layer weights $\frac{\partial \Loss}{\partial \beta_r}$ contains only the local inputs $\psi(w_r x_i)$ and error signal $e_i = f(x_i) - y_i$, while the gradient of first-layer weights $\frac{\partial \Loss}{\partial w_r}$ requires not only the local input $x_i$ and the local output $w_r x_i$ but also the backpropagated error signal $e_i\beta_r$, which contains information on the second-layer feed-forward weight $\beta_r$. This appearance of $\beta_r$ is due to the chain rule between the two adjacent layers and can be recognized as the backward weights in reverse propagation of error signals.
Consequently, backpropagation requires the forward weights between layers to be identical with the backward weights. However, from a biological perspective, this is a requirement on synaptic symmetry and is regarded as too strong to be biological plausible \citep{lillicrap2016random}. 

\paragraph{Feedback alignment on two-layer network.}

One of the alternative approaches proposed to improve the biological plausibility over backpropagation is \emph{Feedback Alignment}, which at the backpropagation stage replaces the forward weights at each layer by an independent fixed random backpropagation weights \citep{lillicrap2016random}. In particular, for the two-layer networks considered in this work, the second-layer weights $\beta$ is replaced by a fixed random backpropagation weights $b\in\Rp$ at backpropagation stage while the gradient update on $\beta$ remains the same, \ie,
\begin{align}\label{eqn:alignment-update}
    \dfa(w_r) = \frac{1}{\sqrt{p}} \sum_{i=1}^n e_i b_r\psi'(w_r\transpose x_i)x_i.
\end{align}
After the substitution, the feedback alignment update on $W(t)$ no longer depends on $\beta(t)$ directly and therefore bears no requirement on synaptic symmetry. Note that the path of $\beta(t)$ does not follow the one by gradient descent under standard backpropagation when considered jointly with the feedback alignment updates on $W(t)$. It is important to notice that the feedback alignment algorithm that we end up arriving at does not explicitly optimize on any particular loss function even though we motivate the algorithm with a loss function $\Loss$ and the corresponding gradient descent algorithm.
In \cref{algo:fa}, we summarize the feedback alignment algorithm on \eqref{eqn:nonlinear-network}.

%\begin{minipage}{\textwidth}
\begin{algorithm}[H]
\centering
\caption{Feedback Alignment on Two-Layer Networks}\label{algo:fa}
    \begin{algorithmic}[1]
        \Require activation $\psi$, dataset $\{(x_i,y_i)\}_{i=1}^n$, and step size $\eta$.
        \State {\bf initialize} $W(0)$, $\beta(0)$ and $b$ with standard Gaussian entries
        \While{not converge}
            \State $\beta_r(t+1) \gets \beta_r(t) - \frac{\eta}{\sqrt p} \sum_{i=1}^n e_i(t)\psi(w_r(t)\transpose x_i)$ for $r\in[p]$
            \State $w_r(t+1) \gets w_r(t) - \frac{\eta}{\sqrt{p}} \sum_{i=1}^n e_i(t) b_r\psi'(w_r(t)\transpose x_i)x_i$ for $r\in[p]$
        \EndWhile
    \end{algorithmic}    
\end{algorithm}%
%\end{minipage}




==> prelim.tex <==
%!TEX root=./main.tex
\section{Preliminaries}

In this paper, we consider a two-layer neural network $f:\Rd \to \RR$ with hidden-layer width $p$. For any input $x\in\Rd$, the network outputs
\begin{align}\label{eqn:nonlinear-network}
    f(x) = \frac{1}{\sqrt p}\sum_{r=1}^p\beta_r\psi(w_r\transpose x)= \frac{1}{\sqrt p}\beta\transpose\psi(Wx),
\end{align}
where $W = (w_1,...,w_p)\transpose\in\Rpd$ and $\beta = (\beta_1,...,\beta_p)\transpose\in\Rp$ represent the feed-forward weights for the first and the second layer, and $\psi$ denotes an element-wise activation function.
Given $n$ input-label pairs $\{(x_i,y_i)\}_{i=1}^n$, we hope to minimize the squared error loss
\begin{equation}\label{eqn:squared-loss}
    \Loss(W,\beta) = \frac{1}{2}\sum_{i=1}^n \big(f(x_i)-y_i\big)^2.
\end{equation}
Vanilla gradient descent minimizes \eqref{eqn:nonlinear-network} through updating the feed-forward weights following gradient directions, \ie,
\begin{align*}
    \beta_r(t+1) = \beta_r(t)-\eta\frac{\partial\Loss}{\partial \beta_r}(W(t),\beta(t)), \quad w_r(t+1) = w_r(t)-\eta\frac{\partial\Loss}{\partial w_r}(W(t),\beta(t)),
\end{align*}
where $\eta>0$ denotes the step size. In this paper, we initialize $\beta(0)$ and $w_r(0)$ for all $r\in[p]$ with standard Gaussian vectors. To simplify the notation, we introduce in the rest of this paper $u(t),e(t)\in \R^n$, where $u_i(t)$ denotes the network output on input $x_i$ at step $t$ and $e_i(t) = u_i(t)-y$ represents the corresponding prediction error.

\paragraph{Backpropagation on two-layer network.}

Backpropagation has been the most commonly used scheme for calculating the gradient of network parameters. In particular, for two-layer network \eqref{eqn:nonlinear-network}, the gradients with respect to the first- and second-layer weights under backpropagation write
\begin{equation*}
    \frac{\partial\Loss}{\partial \beta_r} = \frac{1}{\sqrt p}\sum_{i=1}^n e_i\psi(w_r\transpose x_i), \quad
    \frac{\partial\Loss}{\partial w_r} = \frac{1}{\sqrt p} \sum_{i=1}^n e_i \beta_r\psi'(w_r\transpose x_i)x_i.
\end{equation*}
However, such learning algorithm requires updating its weights with backpropagated error signals that consist of non-local information of weight parameters from top layers. More specifically, given an input $x_i$, the gradient of second-layer weights $\frac{\partial \Loss}{\partial \beta_r}$ contains only the local inputs $\psi(w_r x_i)$ and error signal $e_i = f(x_i) - y_i$, while the gradient of first-layer weights $\frac{\partial \Loss}{\partial w_r}$ requires not only the local input $x_i$ and the local output $w_r x_i$ but also the backpropagated error signal $e_i\beta_r$, which contains information on the second-layer feed-forward weight $\beta_r$. This appearance of $\beta_r$ is due to the chain rule between the two adjacent layers and can be recognized as the backward weights in reverse propagation of error signals.
Consequently, backpropagation requires the forward weights between layers to be identical with the backward weights. However, from a biological perspective, this is a requirement on synaptic symmetry and is regarded as too strong to be biological plausible \citep{lillicrap2016random}. 

\paragraph{Feedback alignment on two-layer network.}

One of the alternative approaches proposed to improve the biological plausibility over backpropagation is \emph{Feedback Alignment}, which at the backpropagation stage replaces the forward weights at each layer by an independent fixed random backpropagation weights \citep{lillicrap2016random}. In particular, for the two-layer networks considered in this work, the second-layer weights $\beta$ is replaced by a fixed random backpropagation weights $b\in\Rp$ at backpropagation stage while the gradient update on $\beta$ remains the same, \ie,
\begin{align}\label{eqn:alignment-update}
    \dfa(w_r) = \frac{1}{\sqrt{p}} \sum_{i=1}^n e_i b_r\psi'(w_r\transpose x_i)x_i.
\end{align}
After the substitution, the feedback alignment update on $W(t)$ no longer depends on $\beta(t)$ directly and therefore bears no requirement on synaptic symmetry. Note that the path of $\beta(t)$ does not follow the one by gradient descent under standard backpropagation when considered jointly with the feedback alignment updates on $W(t)$. It is important to notice that the feedback alignment algorithm that we end up arriving at does not explicitly optimize on any particular loss function even though we motivate the algorithm with a loss function $\Loss$ and the corresponding gradient descent algorithm.
In \cref{algo:fa}, we summarize the feedback alignment algorithm on \eqref{eqn:nonlinear-network}.

%\begin{minipage}{\textwidth}
\begin{algorithm}[H]
\centering
\caption{Feedback Alignment on Two-Layer Networks}\label{algo:fa}
    \begin{algorithmic}[1]
        \Require activation $\psi$, dataset $\{(x_i,y_i)\}_{i=1}^n$, and step size $\eta$.
        \State {\bf initialize} $W(0)$, $\beta(0)$ and $b$ with standard Gaussian entries
        \While{not converge}
            \State $\beta_r(t+1) \gets \beta_r(t) - \frac{\eta}{\sqrt p} \sum_{i=1}^n e_i(t)\psi(w_r(t)\transpose x_i)$ for $r\in[p]$
            \State $w_r(t+1) \gets w_r(t) - \frac{\eta}{\sqrt{p}} \sum_{i=1}^n e_i(t) b_r\psi'(w_r(t)\transpose x_i)x_i$ for $r\in[p]$
        \EndWhile
    \end{algorithmic}    
\end{algorithm}%
%\end{minipage}




==> proofs_linear.tex <==

% \subsection{Convergence on Two-Layer Networks}

% \begin{lemma}
%     If $p = \Omega\big( \frac{n^2\log(2n^2/\delta)}{\lambda_0^2} \big)$, then with probability at least $1-\delta$ we have $\|G(0)-G^\infty\| \leq \frac{\lambda_0}{4}$ and $\lambdamin(G(0)) > \frac{3}{4}\lambda_0$.
% \end{lemma}

% \begin{proof}
%     Recall that the $(i,j)$-th entry of $G(0)$ is
%     \begin{align*}
%         G_{ij}(0) = \frac{1}{p} x_i\transpose x_j \sum_{r=1}^p b_r\beta_r(0)\II\{w_r(0)\transpose x_i\geq 0, w_r(0)\transpose x_j\geq 0\},
%     \end{align*}
%     where $b_r\beta_r(0)\II\{w_r(0)\transpose x_i\geq 0, w_r(0)\transpose x_j\geq 0\}$ are independent from each index $r\in [p]$. By Hoeffding's inequality and the fact that $b_r\beta_r(0)\II\{w_r(0)\transpose x_i\geq 0, w_r(0)\transpose x_j\geq 0\}$ is bounded from $-1$ to $1$ and $|\inner{x_i}{x_j}|\leq 1$ under our assumption,
%     \begin{align*}
%         \prob[ |G_{ij}(0) - G^\infty_{ij}| \geq t ] \leq 2 \exp\left( -\frac{2p^2t^2}{2p} \right) = 2 e^{-pt^2}.
%     \end{align*} 
%     Further, take union bound to get
%     \begin{align*}
%         \prob[ \exists (i,j) \st |G_{ij}(0) - G^\infty_{ij}| \geq t ] \leq 2n^2 e^{-pt^2}.
%     \end{align*}
%     Hence, with probability at least $1-\delta$ it holds for every $(i,j)$-th entry $|G_{ij}(0) - G^\infty_{ij}| \leq \sqrt{\frac{\log(2n^2/\delta)}{p}}$. Consequently, we have with probability at least $1-\delta$ the discrepancy term represented by the spectral norm is bounded by
%     \begin{align*}
%         \|G(0)-G^\infty\|^2 \leq \|G(0)-G^\infty\|_F^2 \leq \frac{n^2\log(2n^2/\delta)}{p},
%     \end{align*}
%     which gives $\|G(0)-G^\infty\| \leq \frac{\lambda_0}{4}$ for any $p \geq \frac{16n^2\log(2n^2/\delta)}{\lambda_0^2}$. By matrix perturbation theory, we have
%     \begin{align*}
%         \lambdamin(G(0)) \geq \lambdamin(G^\infty) - \|G(0)-G^\infty\| \geq \frac{3}{4}\lambda_0.
%     \end{align*}
% \end{proof}

\subsection{Convergence on Two-Layer Linear Networks}

We will provide in this section the proof for the convergence of regularized feedback alignment on two-layer linear networks. We first introduce some notation that will facilitate the proofs.

If $X$ is full rank, the singular value decomposition of $X$ writes $X = U\Sigma V\transpose$, where $\Sigma \in \R^{d\times d}$ is a diagonal matrix with positive diagonal entries. Given the rotational invariant property of Gaussian vectors, we can absorb $V$ into $W$ and, without loss of generality, assume $V = I_d$. 
Moreover, instead of working explicitly on $e(t) = f(t) - y$, we consider the updates on $\theta(t) \defeq X\transpose e(t) = \Sigma U\transpose e(t)$, and similarly we write $\theta_\ast \defeq -X\transpose y$. We start by showing how $\theta(t)$ are updated following the regularized feedback alignment.

\begin{lemma}\label{lem:theta-updates}
    Suppose the network \eqref{eqn:linear-network} is trained on data $(X,y)$ with regularized feedback alignment. Define $s_{t} = \sum_{i=0}^{t} \theta(i)$, $\tilde s_{t} = \sum_{i=0}^{t} \prod_{k=i+1}^t (1-\eta\lambda(k))\theta(i)$ and $u = \frac{1}{\sqrt{p}} W(0)\transpose b$, then $\theta(t)$ follows the iteration update
    \begin{align}\label{eqn:theta-tlam-ordinary}
        \begin{split}
            \theta(t+1) & = \Big((1-\eta\lambda(t))I_d - \prod_{k=0}^t(1-\eta\lambda(k))\frac{\eta}{p}b\transpose\beta(0) \Sigma^2 - \frac{\eta}{p}\Sigma^2 W(0)\transpose W(0) + \frac{\eta^2}{p}\big(u\transpose \tilde{s}(t) \Sigma^2 + \Sigma^2 u s(t-1)\transpose \\
            & \qquad + \Sigma^2 s(t-1)u\transpose\big) - \frac{\eta^3}{p^2}\|b\|^2\big(\sum_{i=0}^t\sum_{j=0}^{i-1} \prod_{k=i+1}^t(1-\eta\lambda(k))\theta(j)\transpose \theta(i) \Sigma^2 + \Sigma^2 s(T)s(t-1)\transpose \big) \Big)\theta(t) + \eta\lambda(t) \theta_\ast.
        \end{split}
    \end{align}
\end{lemma}

\begin{proof}
    With the notation $\theta(t) = X\transpose e(t) = \Sigma U\transpose e(t)$, we replace $X\transpose e(t)$ with $\theta(t)$ and rewrite the updates on $W(t)$ and $\beta(t)$ into 
    \begin{align}\label{eqn:parameter-update-reg}
        W(t+1) = W(t) - \frac{\eta}{\sqrt p}b \theta(t)\transpose, \qquad \beta(t+1) = (1-\eta\lambda(t))\beta(t) - \frac{\eta}{\sqrt p} W(t)\theta(t). 
    \end{align}
    Provided the recursive nature of \cref{eqn:parameter-update-reg}, we represent $W(t)$ with only $W(0)$ and $\theta(i)$ for $i\leq t-1$, \ie,
    \begin{align}\label{eqn:Wt}
        W(t) = W(0) - \frac{\eta}{\sqrt p} \sum_{i=0}^{t-1} b\theta(i)\transpose.
   \end{align}
    Similarly, we can also apply the same argument to $\beta(t)$ and present it as
    \begin{align}\label{eqn:betat}
        \beta(t) &= \prod_{k=0}^{t-1}(1-\eta\lambda(k))\beta(0) - \frac{\eta}{\sqrt p}\sum_{i=0}^{t-1} \prod_{k=i+1}^{t-1}(1-\eta\lambda(k))W(i)\theta(i) \\
        & = \prod_{k=0}^{t-1}(1-\eta\lambda(k))\beta(0) - \frac{\eta}{\sqrt p}\sum_{i=0}^{t-1} \prod_{k=i+1}^{t-1}(1-\eta\lambda(k))\Big( W(0) - \frac{\eta}{\sqrt p} \sum_{j=0}^{i-1} b\theta(j)\transpose\Big) \theta(i) \\
        & = \prod_{k=0}^{t-1}(1-\eta\lambda(k))\beta(0) - \frac{\eta}{\sqrt p}\sum_{i=0}^{t-1} \prod_{k=i+1}^{t-1}(1-\eta\lambda(k))W(0)\theta(i) + \frac{\eta^2}{p}b\sum_{i=0}^{t-1}\sum_{j=0}^{i-1} \prod_{k=i+1}^{t-1}(1-\eta\lambda(k))\theta(j)\transpose\theta(i),
    \end{align}
    where the second equality is due to rewriting $W(i) = W(0) - \frac{\eta}{\sqrt p} \sum_{j=0}^{i-1} b\theta(j)\transpose$. By plugging in \cref{eqn:parameter-update-reg} into the presentation of $e(t+1)$, we can get the iteration updates for all $e(t)$ as 
    \begin{align}\label{eqn:error-iterate}
        \begin{split}
            e(t+1) 
            &=\frac{1}{\sqrt p}X W(t+1)\transpose \beta(t+1) - y \\
            &=\frac{1}{\sqrt p}X (W(t) - \frac{\eta}{\sqrt p}b e(t)\transpose X)\transpose((1-\eta\lambda(t))\beta(t)-\frac{\eta}{\sqrt p} W(t)X\transpose e(t)) - y \\ 
            &=(1-\eta\lambda(t))e(t) - (1-\eta\lambda(t)) \frac{\eta}{p}b\transpose\beta(t) XX\transpose e(t) - \frac{\eta}{p}XW(t)\transpose W(t)X\transpose e(t) \\
            & \qquad + \frac{\eta^2}{p^{3/2}}XX\transpose e(t) b\transpose W(t) X\transpose e(t) - \eta\lambda(t) y, 
        \end{split}
    \end{align}
    where the first equality follows the definition of $e(t+1)$, the second equality follows from \cref{eqn:parameter-update-reg}, and the last equality is due to the fact that $y = (1-\eta\lambda(t))y + \eta\lambda(t) y$. Notice that if we multiply both sides of \cref{eqn:error-iterate} by $X\transpose$, it gives the corresponding iteration updates
    \begin{align}\label{eqn:theta-iterate}
        \theta(t+1) = (1-\eta\lambda(t))\theta(t) - (1-\eta\lambda(t)) \frac{\eta}{p} b\transpose\beta(t) \Sigma^2\theta(t) - \frac{\eta}{p} \Sigma^2 W(t)\transpose W(t)\theta(t) + \frac{\eta^2}{p^{3/2}}\Sigma^2\theta(t) b\transpose W(t) \theta(t) + \eta\lambda(t) \theta_\ast, 
    \end{align}
    where $X = U\Sigma$ and $\theta_\ast = -X\transpose y$. Due to the cleaner form of \cref{eqn:theta-iterate}, we are going to focus primarily on the analysis of $\theta(t)$. Further combining \cref{eqn:Wt,eqn:betat} into \cref{eqn:theta-iterate}, we get
    \begin{align*}
        \theta(t+1) & = (1-\eta\lambda(t))\theta(t) - (1-\eta\lambda(t))\frac{\eta}{p}b\transpose\beta(t) \Sigma^2\theta(t) - \frac{\eta}{p}\Sigma^2 W(t)\transpose W(t)\theta(t) + \frac{\eta^2}{p^{3/2}}\Sigma^2\theta(t) b\transpose W(t) \theta(t) + \eta\lambda(t) \theta_\ast \\
        & = (1-\eta\lambda(t))\theta(t) - \frac{\eta}{p}\Big(\prod_{k=0}^t(1-\eta\lambda(k))b\transpose \beta(0) - \frac{\eta}{\sqrt p} b\transpose W(0)\sum_{i=0}^{t-1}\prod_{k=i+1}^t(1-\eta\lambda(k))\theta(i) \\
        & \qquad  + \frac{\eta^2}{p}\|b\|^2\sum_{i=0}^{t-1}\sum_{j=0}^{i-1}\prod_{k=i+1}^t(1-\eta\lambda(k))\theta(j)\transpose\theta(i) \Big)\Sigma^2\theta(t) \\
        & \qquad - \frac{\eta}{p}\Sigma^2\Big( W(0)\transpose W(0) - \frac{\eta}{\sqrt p}W(0)\transpose b\sum_{i=0}^{t-1}\theta(i)\transpose -\frac{\eta}{\sqrt p}\big(\sum_{i=0}^{t-1}\theta(i)\big)b\transpose W(0) + \frac{\eta^2}{p}\|b\|^2 \big(\sum_{i=0}^{t-1}\theta(i)\big)\big(\sum_{i=0}^{t-1}\theta(i)\big)\transpose\Big)\theta(t) \\
        & \qquad + \frac{\eta^2}{p^{3/2}}\Sigma^2\theta(t)\Big(b\transpose W(0) - \frac{\eta}{\sqrt p}\|b\|^2 \sum_{i=0}^{t-1}\theta(i)\transpose\Big)\theta(t) + \eta\lambda(t) \theta_\ast.
    \end{align*}
    Replacing the corresponding quantities with shorthand $s_{t} = \sum_{i=0}^{t} \theta(i)$, $\tilde s_{t} = \sum_{i=0}^{t} \prod_{k=i+1}^t (1-\eta\lambda(k))\theta(i)$ and $u = \frac{1}{\sqrt{p}} W(0)\transpose b$ to get \cref{eqn:theta-tlam-ordinary}.
\end{proof}

Notice that $\lambda(t)$ almost always appears together with $\eta$ in \cref{eqn:theta-tlam-ordinary}, we write $\tilde{\lambda}_t \defeq \eta\lambda(t)$ to lift the burden on our notation. With \cref{eqn:theta-tlam-ordinary} at hand, we show in \cref{thm:convergence} a recursive inequality that characterizes an upper bound on $\|\theta(t)\|$ and how it is related to the regularization $\lambda(t)$.
 
\begin{theorem}\label{thm:convergence}
    Define $S_\lambda\defeq\sum_{t=0}^\infty\lambda(t)$. If $n \geq \frac{1}{\eps\gamma} (d\log\frac{C}{\eps} + \log\frac{1}{\delta})$, $\eps \leq \min\{C,\frac{1}{8}\}$, $\eta\leq \min\{1/(\max_t\lambda(t) + \frac{n}{d}),\frac{1}{2}\}$, $S_\lambda\leq \frac{1}{\eta\sqrt{d}}\sqrt{p}$, and
    \begin{align*}
        p \geq \max\left\{2\log\frac{2d}{\delta},\frac{1}{\eps\gamma} \Big(d\log\frac{C}{\eps} - \log\frac{\delta}{2}\Big),1280(1+\eps)^3d \Big(1+\sqrt{8\log\frac{2d}{\delta}}\Big)^2\right\},
    \end{align*}
    then the following inequality holds for all $t\geq 0$ with probability at least $1-5\delta$:
        \begin{align}\label[ineqn]{ineqn:norm-theta-bound-ordinary}
            \|\theta(t+1)\| \leq \Big(1-\frac{n\eta}{2d}-\tlam(t) \Big)\|\theta(t)\| + \tlam(t)\|\theta_\ast\|. 
        \end{align}
\end{theorem}

\begin{proof}
    We show \cref{ineqn:norm-theta-bound-ordinary} by induction. Assume that \eqref{ineqn:norm-theta-bound-ordinary} holds for all $t=0,\ldots,T$, then for any $t\leq T$, we apply \cref{ineqn:norm-theta-bound-ordinary} repeatedly on the right hand side of itself to get
\begin{align}\label[ineqn]{ineqn:norm-theta-bound-recursive}
    \|\theta(t)\|\leq \prod_{i=0}^{t-1}\Big(1-\frac{n\eta}{2d}-\tlam(i)\Big)\|\theta(0)\| + \sum_{i=0}^{t-1}\tlam(i)\Big(1-\frac{n\eta}{2d}-\tlam(i+1)\Big)\dots \Big(1-\frac{n\eta}{2d}-\tlam(i-1)\Big)\|\theta_\ast\|.
\end{align}
Notice that $\|s(T)\| \leq \sum_{i=0}^T \|\theta(t)\|$, and $\sum_{i=0}^T \|\theta(t)\|$ can be bounded by summing up both sides of \cref{ineqn:norm-theta-bound-recursive}:
\begin{align}
    \sum_{t=0}^T \|\theta(t)\|
    &\leq  \sum_{t=0}^T\prod_{i=0}^{t-1}\Big(1-\frac{n\eta}{2d}-\tlam(i)\Big)\|\theta(0)\| + \sum_{t=0}^T\sum_{i=0}^{t-1}\tlam(i)\Big(1-\frac{n\eta}{2d}-\tlam(i+1)\Big) \cdots \Big(1-\frac{n\eta}{2d}-\tlam(i-1)\Big)\|\theta_\ast\| \nonumber \\
    &\leq \sum_{t=0}^T\prod_{i=0}^{t-1}\Big(1-\frac{n\eta}{2d}\Big)\|\theta(0)\|+\sum_{t=0}^T\sum_{i=0}^{t-1}\tlam(i)\Big(1-\frac{n\eta}{2d}\Big)^{t-i-1}\|\theta_\ast\| \nonumber \\
    &\leq \sum_{t=0}^T\Big(1-\frac{n\eta}{2d}\Big)^{t-1}\|\theta(0)\| + \|\theta_\ast\|\sum_{i=0}^{t-1}\tlam(i)\sum_{t=i+1}^T \Big(1-\frac{n\eta}{2d}\Big)^{t-i-1} \nonumber \\
    &\leq \frac{2d}{n\eta}\|\theta(0)\| + \frac{2d}{n} S_\lambda\|\theta_\ast\|, \label[ineqn]{ineqn:sum-theta-norm}
\end{align}
where the second inequality follows from $0\leq \tlam(i) = \eta\lambda(i) \leq 1-\frac{n\eta}{d} < 1-\frac{n\eta}{2d}$ for all $i\in[T]$, the third inequality is due to switching the order of summations on running indices $t$ and $i$, and the last inequality is due to $\sum_{t=i+1}^T (1-\frac{n\eta}{2d})^{t-i-1} \leq \sum_{t=0}^T(1-\frac{n\eta}{2d})^{t-1} \leq \sum_{t=0}^\infty (1-\frac{n\eta}{2d})^{t-1} \leq \frac{2d}{n\eta}$ and $\frac{1}{\eta}\sum_{i=0}^{t-1}\tlam(i) \leq S_\lambda$.

Recall that $\theta(t)$ evolves following \cref{eqn:theta-iterate}.
To lift some burden on our notation, we define the following matrices
\begin{align*}
    \Delta(t) \defeq \frac{\eta^2}{p^2} \|b\|^2\big(\sum_{i=0}^t\sum_{j=0}^i \prod_{k=i+1}^t(1-\eta\lambda(k))\theta(j)\transpose \theta(i) \Sigma^2 + \Sigma^2 s(T) s(t-1)\transpose \big)
\end{align*}
and
\begin{align*}
    \Xi(t) \defeq \frac{\eta}{\sqrt p}\big(u\transpose \tilde{s}(t) \Sigma^2 + \Sigma^2 u s(t-1)\transpose + \Sigma^2 s(t-1)u\transpose\big).
\end{align*}
Consequently, \cref{eqn:theta-tlam-ordinary} admits a more concise representation
\begin{align*}
    \begin{split}
        \theta(t+1) & = \Big((1-\tlam(t))I_d -\prod_{k=0}^T(1-\tlam(k))\frac{\eta}{p}b\transpose\beta(0) \Sigma^2 - \frac{\eta}{p}\Sigma^2 W(0)\transpose W(0) + \frac{\eta}{\sqrt p}\Xi(t) - \eta\Delta(t) \Big)\theta(t) + \tlam(t) \theta_\ast \\
        & = \Big( \frac{\eta}{\sqrt p}\Xi(t) - \eta\Delta(t) - \prod_{k=0}^T (1-\tlam(k)) \frac{\eta}{p} b\transpose\beta(0) \Sigma^2 + \frac{n\eta}{d}I_d - \frac{\eta}{p}\Sigma^2 W(0)\transpose W(0) \Big)\theta(t) \\
        & \qquad + \Big( 1-\tlam(t) - \frac{n\eta}{d} \Big)\theta(t) + \tlam(t) \theta_\ast,
    \end{split}
\end{align*}
and triangular inequality and Cauchy-Schwarz inequality give us an upper bound on $\|\theta(t+1)\|$, \ie,
\begin{align}\label[ineqn]{ineqn:theta-upper-bound}
    \begin{split}
        \|\theta(t+1)\| & \leq \left\| \Big( \frac{\eta}{\sqrt p}\Xi(t) - \eta\Delta(t) - \prod_{k=0}^T(1-\tlam(k))\frac{\eta}{p}b\transpose\beta(0) \Sigma^2 + \frac{n\eta}{d}I_d - \frac{\eta}{p}\Sigma^2 W(0)\transpose W(0) \Big)\theta(t) \right\| \\
        & \qquad + \Big( 1-\tlam(t) - \frac{n\eta}{d} \Big)\|\theta(t)\| + \tlam(t) \|\theta_\ast\| \\
        & \leq \eta \Big( \|\Delta(t)\| + \frac{1}{\sqrt p}\|\Xi(t)\| + \frac{1}{p}|b\transpose\beta(0)| \|\Sigma^2\| + \Big\| \frac{n}{d}I_d - \frac{1}{p}\Sigma^2 W(0)\transpose W(0) \Big\| \Big) \|\theta(t)\| \\
        & \qquad + \Big( 1-\tlam(t) - \frac{n\eta}{d} \Big)\|\theta(t)\| + \tlam(t) \|\theta_\ast\|.
    \end{split}
\end{align}
By \cref{cor:b-norm-concentration,cor:W0-b-tail,cor:W0-tail,lem:inner-product-tail}, for any $\eps \leq C$, $n \geq \frac{1}{\eps\gamma} (d\log\frac{C}{\eps} + \log\frac{1}{\delta})$, and
\begin{align*}
    p \geq \max\left\{128\log\frac{2}{\delta},2\log\frac{2d}{\delta},\frac{1}{\eps\gamma} \Big(d\log\frac{C}{\eps} - \log\frac{1}{\delta}\Big)\right\},
\end{align*}
the following inequalities hold with probability at least $1-4\delta$:
\begin{gather*}
    \|b\|^2 \leq \left(1 + \frac{4}{\sqrt p}\sqrt{\log\frac{2}{\delta}}\right) p, \quad \|u\| \leq \sqrt{8d\log\frac{2d}{\delta}}, \quad \frac{|\inner{b}{\beta(0)}|}{\sqrt{p}} \leq \sqrt{8\log\frac{2}{\delta}}, \\ 
    \Big\| \frac{d}{np}X\transpose XW(0)\transpose W(0) - I_d \Big\| \leq \varepsilon, \quad \|\theta(0)\|\leq (1+\eps)\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\frac{n}{\sqrt{d}}, \quad \|\theta_*\|\leq (1+\eps)\frac{n}{\sqrt{d}}.
\end{gather*}
In particular, we use them to upper bound the right-hand side of \cref{ineqn:theta-upper-bound}. Note that if $p\geq 1280(1+\eps)^3d(1+\sqrt{8\log\frac{2d}{\delta}})^2$ and $S_\lambda\leq \frac{1}{\eta\sqrt{d}}\sqrt{p}$, it holds that
\begin{align}\label[ineqn]{ineqn:bound-delta-ordinary}
    \begin{split}
        \|\Delta(t)\| & \leq \frac{2(1+\eps)n\eta^2}{dp} \left(1 + \frac{4}{\sqrt p}\sqrt{\log\frac{2}{\delta}}\right) \Big(\sum_{t=0}^T\|\theta(t)\|\Big)^2 \\
        & \leq \frac{8(1+\eps)d}{np} \left(1 + \frac{4}{\sqrt p}\sqrt{\log\frac{2}{\delta}}\right) (\|\theta(0)\|+ \eta S_\lambda\|\theta_\ast\|)^2 \\
        & \leq  \frac{16(1+\eps)d}{np} \left(1 + \frac{4}{\sqrt p}\sqrt{\log\frac{2}{\delta}}\right) (\|\theta(0)\|^2 + \eta^2 S_\lambda^2\|\theta_\ast\|^2) \\
        & \leq \frac{n}{16d} + \frac{n}{16d}.
    \end{split}
\end{align}
Similarly, if $p\geq 96(1+\eps)^2 d\sqrt{8\log\frac{2d}{\delta}}(1 + \sqrt{8\log\frac{2d}{\delta}})$ and $S_\lambda\leq \frac{1}{\eta d\sqrt{8\log\frac{2d}{\delta}}}p$, it holds that
\begin{align}\label[ineqn]{ineqn:bound-uS-ordinary}
    \begin{split}
        \frac{1}{\sqrt p}\|\Xi(t)\| & \leq \frac{3(1+\eps)n\eta}{dp} \|u\|\|s(T)\| \\
        & \leq \frac{6(1+\eps)}{p} \sqrt{8d\log\frac{2d}{\delta}} (\|\theta(0)\|+ \eta S_\lambda\|\theta_\ast\|) \\
        & \leq \frac{n}{16d} + \frac{n}{16d}.
    \end{split}
\end{align}
Further, following the assumptions that $\eps \leq \min\{C,\frac{1}{8}\}$ and $p\geq 128\log\frac{2}{\delta}\geq 64(1+\eps)^2\log\frac{2}{\delta}$, we have
\begin{align}\label[ineqn]{ineqn:bound_b_beta_ordinary}
    \begin{split}
        \frac{1}{p}|b\transpose\beta(0)| \|\Sigma^2\| & \leq \frac{(1+\eps)n}{d\sqrt p}\sqrt{8\log\frac{2}{\delta}} \leq \frac{(1+\eps)}{\sqrt p}\sqrt{8\log\frac{2}{\delta}} \cdot \frac{n}{d} \leq \frac{n}{8d}
    \end{split}
\end{align}
and
\begin{align}\label[ineqn]{ineqn:bound-XW-ordinary}
    \begin{split}
        \Big\| \frac{n}{d}I_d - \frac{1}{p}\Sigma^2 W(0)\transpose W(0) \Big\| \leq \frac{n}{d}\eps\leq \frac{n}{8d}.
    \end{split}
\end{align}
Combine \cref{ineqn:theta-upper-bound,ineqn:bound-delta-ordinary,ineqn:bound-uS-ordinary,ineqn:bound_b_beta_ordinary,ineqn:bound-XW-ordinary} to get the desired upper bound 
\begin{align*}
    \|\theta(t+1)\| & \leq \Big( 1-\tlam(t) - \frac{n\eta}{d} \Big) \|\theta(t)\| + \eta \Big(  \frac{n}{8d}+ \frac{n}{8d}+ \frac{n}{8d}+ \frac{n}{8d}\Big) \|\theta(t)\|+ \tlam(t)\|\theta_\ast\| \\
    & = (1-\frac{n\eta}{2d}-\tlam(t))\|\theta(t)\|+ \tlam(t)\|\theta_\ast\|.
\end{align*}
\end{proof}

\begin{corollary}\label{cor:convergence}
    If we assume all the conditions from Theorem \ref{thm:convergence}, the prediction error $\|e(t)\|^2$ under feedback alignment based on loss function \eqref{eqn:loss-with-reg} achieves an $O(1/t)$ convergence rate. In particular, with probability at least $1-5\delta$ that 
    \begin{align*}
        \min_{t\leq T}\|\theta(t)\| \leq \frac{2(1+\eps)\sqrt{d}}{(T+1)\eta} \Big( \Big(1 + \sqrt{8\log\frac{2d}{\delta}}\Big) + \frac{1}{\sqrt{d}}\sqrt{p} \Big).
    \end{align*}
\end{corollary}

\begin{proof}
    From Theorem \ref{thm:convergence}, we have $\|\theta(t+1)\| \leq (1-\frac{n\eta}{2d}-\tlam(t))\|\theta(t)\| + \tlam(t)\|\theta_\ast\|$ for all $t\geq 0$. Sum up both sides of the inequality from $0$ to $T$ and rearrange the terms to get
    \begin{align*}
        \min_{t\leq T} \|\theta(t)\|\sum_{t=0}^T \Big(\frac{n\eta}{2d}+\tlam(t)\Big) \leq \sum_{t=0}^T \Big(\frac{n\eta}{2d}+\tlam(t)\Big)\|\theta(t)\| \leq \sum_{t=0}^T (\|\theta(t)\|- \|\theta(t+1)\|) + \sum_{t=0}^T \tlam(t)\|\theta_\ast\|.
    \end{align*}
    Divide the sum $\sum_{t=0}^T (\frac{n\eta}{2d}+\tlam(t))$ on both sides and simplify the telescope sum on the right-hand side, we conclude that
    \begin{align*}
        \min_{t\leq T}\|\theta(t)\| & \leq \frac{\|\theta(0)\| - \|\theta(t+1)\|}{\sum_{t=0}^T (\frac{n\eta}{2d}+\tlam(t))} + \frac{\sum_{t=0}^T \tlam(t)\|\theta_\ast\|}{\sum_{t=0}^T (\frac{n\eta}{2d}+\tlam(t))} \\
        & \leq \frac{2d\|\theta(0)\|}{(T+1)n\eta} + \frac{2d\sum_{t=0}^T \tlam(t)\|\theta_\ast\|}{(T+1)n\eta} \\
        & \leq \frac{2d\|\theta(0)\|}{(T+1)n\eta} + \frac{2d S_\lambda\|\theta_\ast\|}{(T+1)n} \\
        & \leq \frac{2(1+\eps)\sqrt{d}}{(T+1)\eta} \Big( \Big(1 + \sqrt{8\log\frac{2d}{\delta}}\Big) + \frac{1}{\sqrt{d}}\sqrt{p} \Big),
    \end{align*}
    where the second inequality is due to $\|\theta(0)\| - \|\theta(t+1)\| \leq \|\theta(0)\|$ and $(T+1)\frac{n\eta}{2d} \leq \sum_{t=0}^T (\frac{n\eta}{2d}+\tlam(t))$, and the second inequality is due to $\eta S_\lambda = \sum_{t=0}^T \tlam(t)$, and the last inequality is due to the conditions from Theorem \ref{thm:convergence}.
\end{proof}

\begin{corollary}\label{cor:convergence-without-reg}
    If we assume all conditions from Theorem \ref{thm:convergence}, the prediction error $\|e(t)\|$ under feedback alignment on \eqref{eqn:loss-with-reg} without regularization, \ie, $\lambda(t) = 0$, achieves linear convergence rate. In particular, $\|e(t)\| \leq \frac{1+\eps}{1-\eps}(1-\frac{n\eta}{2d})^t \|e_0\|$.
\end{corollary}

\begin{proof}
    Without regularization, \cref{ineqn:norm-theta-bound-ordinary} can be reduced to $\|\theta(t+1)\| \leq (1-\frac{n\eta}{2d}) \|\theta(t)\|$, and consequently we have
    \begin{align*}
        \|\theta(t)\| \leq \Big(1-\frac{n\eta}{2d}\Big)^t \|\theta(0)\|.
    \end{align*}
    Recall that $\theta(t) = X\transpose e(t) = \Sigma U\transpose e(t)$ and $1-\eps\leq \lambda_\mmin(\Sigma)\leq \lambda_\mmax(\Sigma)\leq 1+\eps$ with probability at least $1-\delta$. Hence, we have $\|e(t)\|$ also converging at linear rate for any $e_0$ in the column space of $X$.
\end{proof}

\begin{corollary}\label{cor:convergence-with-decreasing-reg}
    If we assume all conditions from Theorem \ref{thm:convergence}, the prediction error $\|e(t)\|$ under feedback alignment on \eqref{eqn:loss-with-reg} with regularization $\lambda(t) = \left(1-\frac{\eta\sqrt{d}}{\sqrt{p}}\right)^t$ and $p \geq \frac{8d^2\sqrt{d}}{n^2\eta}$ achieves linear convergence rate. In particular, for $t\geq \icomment{TODO}$, $\|e(t)\| \leq \icomment{TODO}$.
\end{corollary}

\begin{proof}
    Recall from Theorem \ref{thm:convergence} that 
    \begin{align*}
        \|\theta(t+1)\| \leq \Big(1-\frac{n\eta}{2d}- \lambda(t)\eta \Big)\|\theta(t)\| + \lambda(t)\eta\|\theta_\ast\| \leq \Big(1-\frac{n\eta}{2d} \Big)\|\theta(t)\| + \lambda(t)\eta\|\theta_\ast\|,
    \end{align*}
    where the second inequality follows from $\lambda(t)\geq 0$. Equivalently, we can obtain the following upper bound for $\|\theta(t+1)\|$ by recursion:
    \begin{align*}
        \|\theta(t+1)\| \leq \lambda(t)\eta \|\theta_*\| + \sum_{i=1}^t \Big( 1-\frac{n}{2d}\eta \Big)^{t-i} \lambda(i)\eta \|\theta_*\| + \Big( 1-\frac{n}{2d}\eta \Big)^t \|\theta(0)\|,
    \end{align*}
    where the last term on the right-hand side goes to zero as $t\to\infty$. In particular, if $p \geq \frac{8d^2\sqrt{d}}{n^2\eta}$, then it holds that $\left( 1-\frac{n}{2d}\eta \right)^t \|\theta(0)\| \leq \frac{1}{2} \left( 1-\frac{\eta\sqrt{d}}{\sqrt{p}} \right)^t \eta \|\theta_*\| = \frac{1}{2}\lambda(t)\eta \|\theta_*\|$ for any 
    \begin{align*}
        t \geq \log\frac{2\|\theta(0)\|}{\eta\|\theta_*\|} / \log \frac{1-\frac{\eta\sqrt{d}}{\sqrt{p}}}{1 - \frac{n}{2d}\eta}.
    \end{align*}
    Further, note that 
    \begin{align*}
        \sum_{i=1}^t \Big( 1-\frac{n}{2d}\eta \Big)^{t-i} \lambda(i)\eta \|\theta_*\| & = \sum_{i=1}^t \Big( 1-\frac{n}{2d}\eta \Big)^{t-i} \left(1-\frac{\eta\sqrt{d}}{\sqrt{p}}\right)^i \eta \|\theta_*\| \\
        & \leq (t-1) \left(1-\frac{\eta\sqrt{d}}{\sqrt{p}}\right)^t \eta \|\theta_*\| \\
        & = (t-1)\lambda(t)\eta \|\theta_*\|,
    \end{align*}
    where the inequality is due to $\frac{\eta\sqrt{d}}{\sqrt{p}} \leq \frac{1}{2}\frac{n}{2d}\eta$. Combining the inequalities above to get
    \begin{align*}
        \|\theta(t)\| & \leq  \lambda(t)\eta \|\theta_*\| + (t-1)\lambda(t)\eta \|\theta_*\| + \frac{1}{2}\lambda(t)\eta \|\theta_*\| \\
        & \leq 2(t-1) \left(1-\frac{\eta\sqrt{d}}{\sqrt{p}}\right)^{t-1} \eta \|\theta_*\| \\
        & \leq 
    \end{align*}
\end{proof}

\begin{lemma}\label{lem:series}
    If a number series $\{x_t\}_{t=0}^\infty$ is subjected to $x_{t+1} = (1-a)x_t + b$, where $x_t > 0$ and $a\in(0,1)$, it holds $x_{t+1} - \frac{b}{a} = (1-a) (x_t - \frac{b}{a})$, and $x_n$ converges to $x_\infty = \frac{b}{a}$ exponentially fast. In particular, for any $\eps >0$, we have $|x_t-x_\infty|<\eps$ for any $t = \Omega(\frac{1}{a}\log\frac{1}{\eps})$.
\end{lemma}

\begin{lemma}\label{lem:series-bound}
   For orthogonal decomposition $\theta(t) = a(t) \hat\theta_\ast + \Xi(t)$, where $\hat\theta_\ast = \theta_\ast/\|\theta_\ast\|$ and $\Xi(t) \perp \theta_\ast$, if we assume the conditions of \cref{cor:W0-tail} with regularization $\lambda(t) = \lambda$ for the first $T$ steps and $\lambda \geq \frac{4n}{d}$, then if it holds $\eps\leq \frac{1}{40}$,
   \begin{align*}
       p\geq \max\left\{2048\log\frac{2}{\delta},2560(1+\eps)^3d(1+\sqrt{8\log\frac{2d}{\delta}})^2\right\}
   \end{align*}
   and $S_\lambda = T\lambda\leq \frac{1}{\eta\sqrt{d}}\sqrt{p}$, then for any $\delta>0$, there exists
   \begin{align*}
       \tau & = \Bigg[\log\left(\frac{\lambda+\frac{n}{2d}}{\frac{n}{2d}\|\theta_*\|} \left(\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\frac{(1+\eps)n}{\sqrt{d}} - \frac{(1+\eps)\lambda}{\lambda + \frac{n}{2d}}\frac{n}{\sqrt{d}}\right)\right) + \log\frac{\lambda}{\frac{n}{2d}} + \log\frac{\lambda-\frac{n}{d}}{\frac{n}{d}}\Bigg]/\log\frac{1}{1 - (\lambda+\frac{n}{2d})\eta},
   \end{align*}
   such that for any $t>\tau$, we have $a(t)\geq \frac{(\lambda - \frac{2n}{d})\|\theta_*\|}{\lambda + \frac{n}{d}}$ and $\|\Xi(t)\|\leq \frac{\frac{n}{d}\|\theta_*\|}{\lambda + \frac{n}{2d}}$ with probability at least $1-5\delta$.
\end{lemma}

\begin{proof}
    Multiply $\hat\theta_\ast$ on both sides of \cref{eqn:theta-tlam-ordinary} to get the iterate for $a(t)$:
    \begin{align}\label{eqn:a(t)lam-ordinary}
        \begin{split}
            a(t+1) & = \Big((1-\tlam(t))I_d -\prod_{k=0}^t(1-\tlam(k))\frac{n\eta}{dp}b\transpose\beta(0) I_d -\frac{n\eta}{d} I_d - \frac{n\eta^3}{dp^2}\|b\|^2\big(\sum_{i=0}^t\sum_{j=0}^i\prod_{k=i+1}^t(1-\tlam(k))\theta(j)\transpose \theta(i) I_d \big)\Big) a(t) \\
            & \qquad + \hat\theta_\ast\transpose\Big( \frac{\eta^2}{p}\big(u\transpose \tilde{s}(t) \Sigma^2 + \Sigma^2 u s(t-1)\transpose + \Sigma^2 s(t-1)u\transpose\big) + \eta\Big(\frac{n}{d}I_d - \frac{1}{p}\Sigma^2 W(0)\transpose W(0)\Big) \\
            & \qquad + \prod_{k=0}^t (1-\tilde\lambda(k))\frac{\eta}{p}b\transpose\beta(0) \Big(\frac{n}{d}I_d - \Sigma^2\Big) + \frac{\eta^3}{p^2}\|b\|^2\sum_{i=0}^t\sum_{j=0}^i\prod_{k=i+1}^t(1-\tilde\lambda(k))\theta(j)\transpose \theta(i) \Big(\frac{n}{d}I_d-\Sigma^2\Big) \Big)\theta(t) \\
            & \qquad -\frac{\eta^3}{p^2}\|b\|^2 \hat\theta_\ast\transpose \Sigma^2 s_{t}s(t-1)\transpose \theta(t) + \tlam(t)\|\theta_*\|.
        \end{split}
    \end{align}
    For any $n,d,p$ satisfy the condition of \cref{cor:W0-tail}, if $p\geq \max\{512\log\frac{2}{\delta},1280(1+\eps)^3d(1+\sqrt{8\log\frac{2d}{\delta}})^2\}$ and $S_\lambda\leq \frac{1}{\eta\sqrt{d}}\sqrt{p}$, it holds with probability at least $1-4\delta$ that $\prod_{k=0}^t (1-\tlam(k))\frac{n\eta}{dp} b\transpose\beta(0) \leq \frac{n\eta}{dp}b\transpose\beta(0) \leq \frac{n\eta}{8d}$,
    \begin{align*}
        \frac{n\eta^3}{dp^2}\|b\|^2 \sum_{i=0}^t\sum_{j=0}^i\prod_{k=i+1}^t(1-\tlam(k))\theta(j)\transpose \theta(i) \leq \frac{n\eta}{16d}, \qquad
        \frac{\eta^3}{p^2}\|b\|^2 \Sigma^2 s_{t}s(t-1)\transpose \leq \frac{n\eta}{16d}.
    \end{align*}
    For any $n,d,p$ satisfy the condition of \cref{cor:W0-tail}, if $\eps\leq \frac{1}{20}$ and $p\geq \max\{512\log\frac{2}{\delta},1280(1+\eps)^3d(1+\sqrt{8\log\frac{2d}{\delta}})^2\}$ and $S_\lambda\leq \frac{1}{\eta\sqrt{d}}\sqrt{p}$, it holds with probability at least $1-5\delta$ that
    \begin{align*}
        \frac{\eta^2}{p}\big(u\transpose \tilde{s}(t) \Sigma^2 + \Sigma^2 u s(t-1)\transpose + \Sigma^2 s(t-1)u\transpose\big) \leq \frac{n\eta}{8d},& \qquad \eta\Big(\frac{n}{d}I_d - \frac{1}{p}\Sigma^2 W(0)\transpose W(0)\Big) \leq \frac{n\eta}{8d}, \\
         \prod_{k=0}^t (1-\tilde\lambda(k))\frac{\eta}{p}b\transpose\beta(0) \Big(\frac{n}{d}I_d - \Sigma^2\Big) \leq \frac{n\eta}{8d},& \qquad \frac{\eta^3}{p^2}\|b\|^2\sum_{i=0}^t\sum_{j=0}^i\prod_{k=i+1}^t(1-\tilde\lambda(k))\theta(j)\transpose \theta(i) \Big(\frac{n}{d}I_d-\Sigma^2\Big) \leq \frac{n\eta}{16d}.
    \end{align*}
    Consequently, it holds for all $t\geq 0$ that 
    \begin{align*}
        a(t+1)\geq \Big(1-\Big(\lambda(t)+\frac{2n}{d}\Big)\eta\Big)a(t)+\lambda(t)\eta\|\theta_*\| - \frac{n\eta}{2d} (|a(t)| + \|\Xi(t)\|)
    \end{align*}
    Similarly, we multiply $\xi_{t+1}$ on both sides of \cref{eqn:theta-tlam-ordinary} to obtain a corresponding upper bound
    \begin{align}\label{eqn:xi_tlam-ordinary}
        \begin{split}
            \|\xi_{t+1}\|^2 & = \Big((1-\tlam(t))I_d -\prod_{k=0}^t(1-\tlam(k))\frac{n\eta}{dp}b\transpose\beta(0) I_d - \frac{n\eta}{d} I_d - \frac{n\eta^3}{dp^2}\|b\|^2\big(\sum_{i=0}^t\sum_{j=0}^i\prod_{k=i+1}^t(1-\tlam(k))\theta(j)\transpose \theta(i) I_d \big)\Big) \xi_{t+1}\transpose \Xi(t) \\
            & \qquad + \xi_{t+1}\transpose\Big(\frac{\eta^2}{p}\big(u\transpose \tilde{s}(t) \Sigma^2 + \Sigma^2 u s(t-1)\transpose + \Sigma^2 s(t-1)u\transpose\big) + \eta\Big(\frac{n}{d}I_d - \frac{1}{p}\Sigma^2 W(0)\transpose W(0)\Big)  \\
            & \qquad + \prod_{k=0}^t(1-\eta\lambda(k))\frac{\eta}{p}b\transpose\beta(0) \Big(\frac{n}{d}I_d - \Sigma^2\Big) + \frac{\eta^3}{p^2}\|b\|^2\sum_{i=0}^t\sum_{j=0}^i\prod_{k=i+1}^t(1-\eta\lambda(k))\theta(j)\transpose \theta(i) \Big(\frac{n}{d}I_d-\Sigma^2\Big) \Big)\theta(t) \\
            & \qquad -\frac{\eta^3}{p^2}\|b\|^2 \xi_{t+1}\transpose \Sigma^2 s(T)s(t-1)\transpose \theta(t) \\
            & \leq \Big(1-\tlam(t)-\frac{3}{4}\frac{n\eta}{d}\Big)\|\xi_{t+1}\| \|\Xi(t)\| - \frac{n\eta}{8d}\|\xi_{t+1}\|\|\theta(t)\| + \frac{n\eta}{32d} \|\xi_{t+1}\|\|\theta(t)\|,
        \end{split}
    \end{align}
    where for any $n,d,p$ satisfy the condition of \cref{cor:W0-tail}, if $\eps\leq \frac{1}{40}$ and $p\geq \max\{2048\log\frac{2}{\delta},2560(1+\eps)^3d(1+\sqrt{8\log\frac{2d}{\delta}})^2\}$ and $S_\lambda\leq \frac{1}{\eta\sqrt{d}}\sqrt{p}$, it holds with probability at least $1-5\delta$ that
    \begin{align*}
        \frac{\eta^2}{p}\big(u\transpose \tilde{s}(t) \Sigma^2 + \Sigma^2 u s(t-1)\transpose + \Sigma^2 s(t-1)u\transpose\big) \leq \frac{n\eta}{16d},& \qquad \eta\Big(\frac{n}{d}I_d - \frac{1}{p}\Sigma^2 W(0)\transpose W(0)\Big) \leq \frac{n\eta}{16d}, \\
        \frac{\eta^3}{p^2}\|b\|^2 \Sigma^2 s_{t}s(t-1)\transpose \leq \frac{n\eta}{32d},& \qquad \frac{\eta^3}{p^2}\|b\|^2\sum_{i=0}^t\sum_{j=0}^i\prod_{k=i+1}^t(1-\tilde\lambda(k))\theta(j)\transpose \theta(i) \Big(\frac{n}{d}I_d-\Sigma^2\Big) \leq \frac{n\eta}{32d},
    \end{align*}
    and 
    \begin{align*}
        \prod_{k=0}^t (1-\tilde\lambda(k))\frac{\eta}{p}b\transpose\beta(0) \Big(\frac{n}{d}I_d - \Sigma^2\Big) \leq \frac{n\eta}{16d}.
    \end{align*}
    In other words, we have $\|\xi_{t+1}\| \leq \big(1-\tlam(t) - \frac{n\eta}{2d})\|\Xi(t)\| + \frac{n\eta}{2d}|a(t)|$ for all $t\geq 0$. Under the assumption that $\lambda > \|\theta(0)\|\geq (1+\eps)(1 + \sqrt{8\log\frac{2d}{\delta}}) \frac{n}{\sqrt{d}}$ with probability at least $1-\delta$, we can rewrite the bounds above for the first $T$ steps into
    \begin{align*}
        \begin{cases}
            a(t+1)\geq (1-(\lambda+\frac{2n}{d})\eta)a(t)+\lambda\eta\|\theta_*\| - \frac{n\eta}{2d} (|a(t)| + \|\Xi(t)\|), \\
            \|\xi_{t+1}\| \leq (1-(\lambda+\frac{n}{2d})\eta)\|\Xi(t)\| + \frac{n\eta}{2d} |a(t)|.
        \end{cases}
    \end{align*}
    Recall that from Theorem \ref{thm:convergence} we have $\|\theta(t+1)\| \leq (1-(\lambda + \frac{n}{2d})\eta )\|\theta(t)\| + \lambda\eta\|\theta_\ast\|$, and we rearrange the terms to get
    \begin{align*}
        \Big(\|\theta(t+1)\| - \frac{\lambda\|\theta_*\|}{\lambda + \frac{n}{2d}}\Big) \leq \Big(1-\Big(\lambda + \frac{n}{2d}\Big)\eta \Big) \Big(\|\theta(t)\|  - \frac{\lambda\|\theta_*\|}{\lambda + \frac{n}{2d}}\Big),
    \end{align*}
    where $\|\theta(t)\|$ converges to $\frac{\lambda\|\theta_*\|}{\lambda + \frac{n}{2d}}$ from above exponentially fast. 
    In particular, for any initialization $\|\theta(0)\| \geq \frac{\lambda\|\theta_*\|}{\lambda + \frac{n}{2d}}$ we have $\|\theta(t)\|\leq \|\theta_*\|$ with probability at least $1-3\delta$ for all $t$ greater than
    \begin{align*}
        \tau_1 & \defeq \log\left(\frac{\lambda+\frac{n}{2d}}{\frac{n}{2d}\|\theta_*\|} \left(\|\theta(0)\| - \frac{\lambda\|\theta_*\|}{\lambda + \frac{n}{2d}}\right)\right)/\log\frac{1}{1 - (\lambda+\frac{n}{2d})\eta} \\
        & \leq \log\left(\frac{\lambda+\frac{n}{2d}}{\frac{n}{2d}\|\theta_*\|} \left(\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\frac{(1+\eps)n}{\sqrt{d}} - \frac{(1+\eps)\lambda}{\lambda + \frac{n}{2d}}\frac{n}{\sqrt{d}}\right)\right)/\log\frac{1}{1 - (\lambda+\frac{n}{2d})\eta}.
    \end{align*}
    Because $|a(t)|\leq \|\theta(t)\|$ for all $t\geq 0$, we further upper bound 
    \begin{align*}
        \|\xi_{t+1}\| \leq \Big(1-\Big(\lambda + \frac{n}{2d}\Big)\eta \Big)\|\Xi(t)\| + \frac{n\eta}{2d}|a(t)| \leq \Big(1-\Big(\lambda + \frac{n}{2d}\Big)\eta \Big)\|\Xi(t)\| + \frac{n\eta}{2d}\|\theta_*\|
    \end{align*}
    for all $t>\tau_1$. 
    Similarly, rearrange the terms to get
    \begin{align*}
        \Big(\|\xi_{t+1}\| - \frac{\frac{n}{2d}\|\theta_*\|}{\lambda + \frac{n}{2d}}\Big) \leq \Big(1-\Big(\lambda + \frac{n}{2d}\Big)\eta \Big) \Big(\|\Xi(t)\| - \frac{\frac{n}{2d}\|\theta_*\|}{\lambda + \frac{n}{2d}}\Big)
    \end{align*}
    where $\|\Xi(t)\|$ converges to $\frac{\frac{n}{2d}\|\theta_*\|}{\lambda + \frac{n}{2d}}$ from above exponentially fast. 
    In particular, if $\lambda\geq \frac{n}{2d}$ we have $\|\Xi(t)\| \leq \frac{\frac{n}{d}\|\theta_*\|}{\lambda + \frac{n}{2d}}$ with probability at least $1-3\delta$ for all $t>\tau_1+\tau_2$ where 
    \begin{align*}
        \tau_2 & \defeq \log \left( \frac{\lambda+\frac{n}{2d}}{\frac{n}{2d}\|\theta_*\|} \frac{\lambda\|\theta_*\|}{(\lambda + \frac{n}{2d})} \right)/\log\frac{1}{1 - (\lambda+\frac{n}{2d})\eta} \\
        & \leq \log\frac{\lambda}{\frac{n}{2d}}/\log\frac{1}{1 - (\lambda+\frac{n}{2d})\eta}.
    \end{align*}
    Finally, for any $t>\tau_1+\tau_2$, it holds $|a(t)|+\|\Xi(t)\|\leq 2\|\theta(t)\|\leq 2\|\theta_*\|$ so that 
    \begin{align*}
        a(t+1)\geq \Big(1-\Big(\lambda + \frac{2n}{d}\Big)\eta \Big)a(t)+\lambda\eta\|\theta_*\| - \frac{n\eta}{2d} \big(|a(t)| + \|\Xi(t)\|\big)
        \geq  \Big(1-\Big(\lambda + \frac{2n}{d}\Big)\eta \Big)a(t)+\lambda\eta\|\theta_*\| - \frac{n\eta}{d}\|\theta_*\|,
    \end{align*}
    and by similar argument we obtain
    \begin{align*}
        \Big(a(t+1) - \frac{(\lambda - \frac{n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}}\Big) \geq  \Big(1-\Big(\lambda + \frac{2n}{d}\Big)\eta \Big) \Big(a(t) - \frac{(\lambda - \frac{n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}}\Big),
    \end{align*}
    where $a(t)$ converges to $\frac{(\lambda - \frac{n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}}$ from below exponentially fast. 
    As long as we have $\lambda\geq \frac{4n}{d}$, it holds with probability at least $1-3\delta$ for any $t>\tau_1+\tau_2+\tau_3$ that $a(t) \geq \frac{(\lambda - \frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} \geq \|\Xi(t)\|$, where 
    \begin{align*}
        \tau_3 & \defeq \log\left(\frac{\lambda+\frac{2n}{d}}{\frac{n}{d}\|\theta_*\|} \left(\frac{(\lambda - \frac{n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} - a_{\tau_1+\tau_2}\right)\right)/\log\frac{1}{1 - (\lambda+\frac{n}{2d})\eta} \\
        & \leq \log\frac{\lambda-\frac{n}{d}}{\frac{n}{d}}/\log\frac{1}{1 - (\lambda+\frac{n}{2d})\eta}.
    \end{align*}
\end{proof}

\subsection{Alignment on Two-Layer Linear Networks}

In this section, we will show the proofs for the alignment between $\beta(t)$ and $b$ under the regularized feedback alignment with cutoff regularization.

\begin{theorem}\label{thm:alignment}
    If we assume all conditions from \cref{lem:series-bound} \icomment{TODO: some extra conditions here} and the regularization term
    \begin{align*}
        \lambda(t) = 
        \begin{cases}
            \lambda, \quad t\leq T,\\
            0, \quad t > T,
        \end{cases}
    \end{align*}
    where $T = \lfloor \frac{\sqrt{d}}{4\eta n}\sqrt{p} \rfloor$ and $\lambda \geq \frac{12n}{d}$,
    then feedback alignment on \eqref{eqn:loss-with-reg} achieves alignment. In particular, $\lim_{t\to\infty} \cos\angle(b, \beta(t)) = \Theta(1)$.
\end{theorem}

\begin{proof}
    Recall that
    \begin{align*}
        \beta(t) &= \prod_{k=0}^{t-1}(1-\tlam(k))\beta(0) - \frac{\eta}{\sqrt p}\sum_{i=0}^{t-1} \prod_{k=i+1}^{t-1}(1-\tlam(k))W(0)\theta(i) + \frac{\eta^2}{p}b\sum_{i=0}^{t-1}\sum_{j=0}^i\prod_{k=i+1}^{t-1}(1-\tlam(k))\theta(j)\transpose\theta(i)
    \end{align*}
    is composed of three parts, where the first part is a multiple of $\beta(0)$ that is almost orthogonal against $b$ upon random initialization and the third part is a multiple of $b$ that contributes positively to the alignment. To simplify the notation, we define $\phi_{1}(t) \defeq \prod_{k=0}^{t-1}(1-\tlam(k))\beta(0)$, $\phi_{2}(t) \defeq \eta\sum_{i=0}^{t-1} \prod_{k=i+1}^{t-1} (1-\tlam(k))\theta(i)$, and $\phi_{3}(t) \defeq \frac{\eta^2}{\sqrt p} \frac{b}{\|b\|} \sum_{i=0}^{t-1} \sum_{j=0}^i \prod_{k=i+1}^{t-1}(1-\tlam(k)) \theta(j)\transpose\theta(i)$, so that we can rewrite 
    \begin{align*}
        \beta(t) = \phi_{1}(t) + \frac{1}{\sqrt p}W(0) \phi_{2}(t) + \frac{\|b\|}{\sqrt p}\phi_{3}(t).
    \end{align*}
    From \cref{cor:W0-tail} we have $1-\eps\leq \frac{1}{\sqrt p} \|W(0)\| \leq 1+\eps$ and from \cref{cor:b-norm-concentration} that $1-\eps \leq \frac{\|b\|}{\sqrt p} \leq 1+\eps$ with probability at least $1-2\delta$. The cosine value of the angle between $b$ and $\beta(t)$ is given by the normalized inner-product between them, which can be lower bounded through
    \begin{align*}
        \cos\angle(b, \beta(t)) 
        = \frac{b\transpose \beta(t)}{\|b\|\|\beta(t)\|}  = \frac{\big(\frac{b}{\|b\|}\big)\transpose \beta(t)}{\|\beta(t)\|} & \geq \frac{\frac{\|b\|}{\sqrt p}\|\phi_{3}(t)\|-\frac{\|b\transpose W(0)\|}{\|b\|\sqrt p}\|\phi_{2}(t)\| - \|\phi_{1}(t)\|}{\|\phi_{1}(t)\|+\frac{\|W(0)\|}{\sqrt p}\|\phi_{2}(t)\|+\frac{\|b\|}{\sqrt p}\|\phi_{3}(t)\|} \\
        & \geq \frac{(1-\eps)\|\phi_{3}(t)\|-\frac{1}{(1-\eps)\sqrt{p}} \sqrt{8d\log\frac{2d}{\delta}} \|\phi_{2}(t)\| - \|\phi_{1}(t)\|}{\|\phi_{1}(t)\|+(1+\eps)\|\phi_{2}(t)\|+(1+\eps)\|\phi_{3}(t)\|}.
    \end{align*}

    Let us write $\theta(t) = a(t) \hat\theta_\ast + \Xi(t)$, where $\Xi(t)\perp\theta_\ast$ and $\hat\theta_* = \theta_*/\|\theta_*\|$. Notice that $\|\phi_{1}(t)\|$ converges to zero exponentially fast for $t\leq T$. In particular, it holds that $1-\eps \leq \frac{\|b\|^2}{p} \leq 1+\eps$ with probability at least $1-\delta$ and thus
    \begin{align*}
        \|\phi_{1}(t)\| & \leq 2\sqrt p \prod_{k=0}^{t-1}(1-\tlam(k)) \leq 2\sqrt p \exp\Big(-\sum_{k=0}^{t-1}\tlam(k)\Big).
    \end{align*} 
    In large $t$ limit, we have $\lim_{t\to\infty}\|\phi_{1}(t)\| \leq 2\sqrt p \exp(-\eta T\lambda)$. Recall that from \cref{lem:series-bound} we require $S_\lambda\leq \frac{1}{\eta\sqrt{d}}\sqrt{p}$ and $\lambda\geq \frac{4n}{d}$ at the same time, and consequently, it is required that $T\leq \frac{\sqrt{d}}{4\eta n}\sqrt{p}$. To achieve the maximum alignment, we take $T=\lfloor \frac{\sqrt{d}}{4\eta n}\sqrt{p} \rfloor$ for the rest of the proof.
    For the other two terms, we also have the following bounds available:
    \begin{align*}
        \|\phi_{2}(t)\| &\leq \eta\sum_{i=0}^{t-1}\prod_{k=i+1}^{t-1}(1-\tlam(k))\|\theta(i)\| 
        \leq \eta\sum_{i=0}^{t-1}\prod_{k=i+1}^{t-1}(1-\tlam(k))(|a(i)|+\|\xi(i)\|), \\
        \|\phi_{2}(t)\| &\geq \eta\left|\sum_{i=0}^{t-1}\prod_{k=i+1}^{t-1}(1-\tlam(k))a(i)\right|, \\
        \|\phi_{3}(t)\| &= \frac{\eta^2}{\sqrt p}\sum_{i=0}^{t-1}\sum_{j=0}^i\prod_{k=i+1}^{t-1}(1-\tlam(k))\theta(i)\transpose \theta(j) \geq \frac{\eta^2}{\sqrt p}\sum_{i=0}^{t-1}\sum_{j=0}^i\prod_{k=i+1}^{t-1}(1-\tlam(k))(a(i)a(j)-\|\xi(i)\|\|\xi(j)\|).
    \end{align*}
    \cref{lem:series-bound} tells us that for $\tau \leq t \leq T$ and $\lambda \geq \frac{4n}{d}$, it holds that $a(t)\geq \frac{(\lambda - \frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} \geq \frac{\frac{2n}{d}\|\theta_*\|}{\lambda + \frac{2n}{d}}$ and $\|\Xi(t)\|\leq \frac{\frac{n}{d}\|\theta_*\|}{\lambda + \frac{n}{2d}}$.
    For any $T = \lfloor \frac{\sqrt{d}}{4\eta n}\sqrt{p} \rfloor$ and $t>T$, it holds
    \begin{align*}
        \|\phi_{3}(t)\| 
        & = \frac{\eta^2}{\sqrt p}\sum_{i=0}^{\frac{T}{K}-1}\sum_{j=0}^i\prod_{k=i+1}^{\frac{T}{K}-1}(1-\tlam(k))\theta(i)\transpose\theta(j) + \frac{\eta^2}{\sqrt p}\sum_{i=\frac{T}{K}}^{T}\prod_{k=i+1}^{T-1}(1-\tlam(k))\theta(i)\transpose\sum_{j=0}^{i-1} \theta(j) \\
        & \qquad + \frac{\eta^2}{\sqrt p}\sum_{i=T+1}^{t-1}\sum_{j=0}^i\prod_{k=i+1}^{t-1}(1-\tlam(k))\theta(i)\transpose\theta(j) \\
        & \geq \frac{\eta^2}{\sqrt p}\sum_{i=\frac{T}{K}}^{T}\prod_{k=i+1}^{T-1}(1-\lambda\eta)\theta(i)\transpose\sum_{j=0}^{i-1} \theta(j) - \frac{\eta^2}{\sqrt p}\sum_{i=0}^{\frac{T}{K}-1}\sum_{j=0}^i\prod_{k=i+1}^{\frac{T}{K}-1}(1-\tlam(k)) \|\theta(i)\|\|\theta(j)\| \\
        & \qquad + \frac{\eta^2}{\sqrt p}\sum_{i=T+1}^{t-1}\sum_{j=0}^i\prod_{k=i+1}^{t-1}(1-\tlam(k)) \theta(i)\transpose \theta(j),
    \end{align*}
    where the inequality follows from $\theta(i)\transpose\theta(j) \leq \|\theta(i)\|\|\theta(j)\|$. We lower bound $\|\phi_{3}(t)\|$ with three parts, where the last two will turn out to be bounded by quantities independent of $p$. In particular, for the first term we have 
    \begin{align*}
        \frac{\eta^2}{\sqrt p}\sum_{i=\frac{T}{K}}^{T-1}\prod_{k=i+1}^{t-1}(1-\tlam(k))\theta(i)\transpose\sum_{j=0}^{i-1} \theta(j) & = \frac{\eta^2}{\sqrt p} \sum_{i=\frac{T}{K}}^{T-1} (1-\lambda\eta)^{t-i-2} \theta(i)\transpose \cdot \Big( \sum_{j=0}^{\tau-1} \theta(j) + \sum_{j=\tau}^{i-1} \theta(j) \Big),
    \end{align*}
    where the equality follows from $\prod_{k=i+1}^{t-1}(1-\tlam(k)) = (1-\lambda\eta)^{t-i-2}$ and splitting the sum of $\theta(j)$ into two parts at $\tau\leq \frac{T}{K}$ if $\sqrt{p} \geq 8Kn\eta\tau/\sqrt{d}$. 
    Similarly, for any $t>T$ we have the following upper bound
    \begin{align*}
        \|\phi_{2}(t)\| 
        &\leq  \eta\sum_{i=\frac{T}{K}}^{T-1} (1-\lambda\eta)^{T-i-2} \|\theta(i)\| + \eta\sum_{i=0}^{\frac{T}{K}-1}\prod_{k=i+1}^{\frac{T}{K}-1}(1-\tlam(k)) \|\theta(i)\| + \eta\sum_{i=T}^{t-1} \prod_{k=T+1}^{t-1}(1-\tlam(k)) \|\theta(i)\|,
    \end{align*}
    where the inequality follows from the triangular inequality. Here we also chop the sum into three parts, and we will show that the first part dominates. 
    
    In the rest part of this proof, we are going to show that $\|\phi_{2}(t)\|$ can be bounded by a constant multiple of $\|\phi_{3}(t)\|$. Notice that for any $i\geq \frac{T}{K} > \tau$ it holds that 
    \begin{align*}
        \theta(i)\transpose\sum_{j=0}^{i-1} \theta(j) & = \theta(i)\transpose \cdot \Big( \sum_{j=0}^{\tau-1} \theta(j) + \sum_{j=\tau}^{i-1} \theta(j) \Big) \\
        & = (a(i)\hat\theta(i)\transpose + \xi(i))\transpose \cdot \Big( \sum_{j=0}^{\tau-1} (a(j)\hat\theta(j)\transpose + \xi(j)) + \sum_{j=\tau}^{i-1} (a(j)\hat\theta(j)\transpose + \xi(j)) \Big) \\
        & = a(i) \Big( \sum_{j=0}^{\tau-1} a(j) + \sum_{j=\tau}^{i-1} a(j) \Big) + \xi(i)\transpose \Big( \sum_{j=0}^{\tau-1} \xi(j) + \sum_{j=\tau}^{i-1} \xi(j) \Big) \\
        & \geq a(i) \Big( (i-\tau) \frac{(\lambda-\frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} - \tau M \Big) - \|\xi(i)\| \Big( \sum_{j=0}^{\tau-1} \|\xi(j)\| + \sum_{j=\tau}^{i-1} \|\xi(j)\| \Big) \\
        & \geq a(i) \Big( (i-\tau) \frac{(\lambda-\frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} - \tau M \Big) - \|\xi(i)\| \Big( \tau M + (i-\tau) \frac{\frac{n}{d}\|\theta_*\|}{\lambda + \frac{n}{2d}} \Big),
    \end{align*}
    where the first inequality follows from $a(j) \geq \frac{(\lambda-\frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}}$ for any $\tau\leq j\leq T$ and Cauchy-Schwarz inequality, and the second inequality follows from $\|\xi(j)\|\leq \frac{\frac{n}{d}\|\theta_*\|}{\lambda + \frac{n}{2d}}$ for any $\tau\leq j\leq T$. Here $M \defeq \max\left\{\|\theta(0)\|,\frac{\lambda\|\theta_*\|}{\lambda + \frac{n}{2d}}\right\}$, and for any $j\geq 0$, both $a(j)$ and $\|\xi(j)\|$ are dominated by $M$. In particular, with probability at least $1-3\delta$ it holds that 
    \begin{align*}
        \max\left\{\|\theta(0)\|,\frac{\lambda\|\theta_*\|}{\lambda + \frac{n}{2d}}\right\} \leq (1+\eps)\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\frac{n}{\sqrt{d}}, \qquad \|\theta_*\| \geq (1-\eps)\|y\|.
    \end{align*}
    If $\lambda\geq \frac{12n}{d}$ and 
    \begin{align*}
        \sqrt{p} \geq 16\eta K\frac{n^2}{d}(1+\eps) \left(1 + \sqrt{8\log\frac{2d}{\delta}}\right) \max\left\{ \frac{\lambda + \frac{n}{2d}}{\frac{n}{d}\|\theta_*\|}, \frac{2(\lambda + \frac{2n}{d})}{(\lambda-\frac{2n}{d})\|\theta_*\|} \right\} \cdot \tau,
    \end{align*}
    we have 
    \begin{align*}
        (i-\tau) \frac{(\lambda-\frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} - \tau M \geq \frac{i}{2} \frac{(\lambda-\frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}}, \qquad \tau M + (i-\tau) \frac{\frac{n}{d}\|\theta_*\|}{\lambda + \frac{n}{2d}} \leq 2i \frac{\frac{n}{d}\|\theta_*\|}{\lambda + \frac{n}{2d}},
    \end{align*}
    and consequently it holds
    \begin{align*}
        \theta(i)\transpose\sum_{j=0}^{i-1} \theta(j) & \geq \frac{i}{2} \frac{(\lambda-\frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} a(i) - 2i \frac{\frac{n}{d}\|\theta_*\|}{\lambda + \frac{n}{2d}} \frac{1}{2}a(i) \\
        & \geq \frac{T}{K} \frac{(\lambda-\frac{10n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} a(i) \\
        & \geq \frac{\|\theta_*\|}{7} \frac{\sqrt{d}}{16\eta n}\sqrt{p} \cdot \frac{2\sqrt{5}}{5}\|\theta(i)\|,
    \end{align*}
    where the first inequality follows from $\|\xi(i)\|\leq \frac{1}{2}a(i)$ for $\tau\leq i\leq T$, the second inequality is due to $\frac{\frac{n}{2d}\|\theta_*\|}{\lambda + \frac{n}{2d}} \leq \frac{\frac{2n}{d}\|\theta_*\|}{\lambda + \frac{2n}{d}}$ and $i\geq \frac{T}{K}$, and the last inequality is due to $T\geq \frac{\sqrt{d}}{8\eta n}\sqrt{p}$, $\lambda\geq \frac{12n}{d}$, and $\|\theta(i)\|\leq \frac{\sqrt{5}}{2}a(i)$ due to the condition $a(i)\geq 2\|\xi(i)\|$ holding for $\tau\leq i\leq T$. Hence, we sum up along the index $i$ to get
    \begin{align*}
        \frac{\eta^2}{\sqrt p}\sum_{i=\frac{T}{K}}^{T-1}\prod_{k=i+1}^{T-1}(1-\tlam(k))\theta(i)\transpose\sum_{j=0}^{i-1} \theta(j) & \geq \frac{\eta^2}{\sqrt p}\sum_{i=\frac{T}{K}}^{T-1}\prod_{k=i+1}^{T-1}(1-\tlam(k)) \frac{\|\theta_*\|}{7} \frac{\sqrt{d}}{16\eta n}\sqrt{p} \cdot \frac{2\sqrt{5}}{5}\|\theta(i)\| \\
        & \geq \eta \frac{\sqrt{5}\|\theta_*\|}{280}\frac{\sqrt{d}}{n} \sum_{i=\frac{T}{K}}^{T-1}\prod_{k=i+1}^{T-1}(1-\tlam(k)) \|\theta(i)\| \\
        & \geq \frac{\sqrt{5}(1-\eps)\|y\|}{280}\frac{\sqrt{d}}{n} \cdot \eta\sum_{i=\frac{T}{K}}^{T-1}(1-\lambda\eta)^{T-i-2} \|\theta(i)\| \\
        & \geq \frac{\sqrt{5}(1-\eps)}{560} \cdot \eta\sum_{i=\frac{T}{K}}^{T-1}(1-\lambda\eta)^{T-i-2} \|\theta(i)\|. \icomment{Require lower bound on $\|\theta_*\|$}
    \end{align*}
    
    Moreover, we could upper bound
    \begin{align*}
        \eta\sum_{i=0}^{\frac{T}{K}-1}\prod_{k=i+1}^{\frac{T}{K}-1}(1-\tlam(k)) \|\theta(i)\| & = \eta\sum_{i=0}^{\tau-1}\prod_{k=i+1}^{\tau-1}(1-\tlam(k)) \|\theta(i)\| + \eta\sum_{i=\tau}^{\frac{T}{K}-1}\prod_{k=i+1}^{\frac{T}{K}-1}(1-\tlam(k)) \|\theta(i)\| \\
        & \leq \eta\tau M + \eta\sum_{i=\tau}^{\frac{T}{K}-1}(1 - \lambda\eta)^{\frac{T}{K}-i-2} \|\theta_*\| \\
        & \leq \eta\tau M + \frac{1}{\lambda} \|\theta_*\|,
    \end{align*}
    where the first inequality follows from $\|\theta(i)\|\leq M$ for all $i\geq 0$ and $\|\theta(i)\|\leq \|\theta_*\|$ for all $\tau\leq i\leq T$, and the second inequality follows from an infinite sum of a geometric series. Similarly, we have
    \begin{align*}
        \eta\sum_{i=T}^{t-1} \prod_{k=T+1}^{t-1}(1-\tlam(k)) \|\theta(i)\| & = \eta\sum_{i=T}^{t-1} \|\theta(i)\| \\
        & \leq \eta \sum_{i=T}^{t-1} \left( 1-\frac{n\eta}{2d} \right)^{i-T} \|\theta(t)\| \\
        & \leq \frac{2d}{n} \|\theta(t)\|,
    \end{align*}
    where the equality is due to $\lambda(k) = 0$ for all $k > T$, the first inequality is due to \cref{cor:convergence}, and the last inequality follows from an infinite sum of geometric series. For the components of $\|\phi_{3}(t)\|$, we also have upper bound 
    \begin{align*}
        & \frac{\eta^2}{\sqrt p}\sum_{i=0}^{\frac{T}{K}-1}\sum_{j=0}^i\prod_{k=i+1}^{\frac{T}{K}-1}(1-\tlam(k)) \|\theta(i)\|\|\theta(j)\| \\
        & = \frac{\eta^2}{\sqrt p}\sum_{i=0}^{\frac{T}{K}-1}(1 - \lambda\eta)^{\frac{T}{K}-i-2} \|\theta(i)\| \sum_{j=0}^i \|\theta(j)\| \\
        & = \frac{\eta^2}{\sqrt p}\sum_{i=0}^{\tau-1}(1 - \lambda\eta)^{\tau-i-2} \|\theta(i)\| \sum_{j=0}^i \|\theta(j)\| + \frac{\eta^2}{\sqrt p}\sum_{i=\tau}^{\frac{T}{K}-1}(1 - \lambda\eta)^{\frac{T}{K}-i-2} \|\theta(i)\| \sum_{j=0}^i \|\theta(j)\| \\
        & \leq \frac{\eta^2}{\sqrt p} \tau^2 M^2 + \frac{\eta^2}{\sqrt p}\sum_{i=\tau}^{\frac{T}{K}-1}(1 - \lambda\eta)^{\frac{T}{K}-i-2} \|\theta(i)\| \Big( \sum_{j=0}^{\tau-1} M + \sum_{j=\tau}^{i} \|\theta_*\| \Big) \\
        & \leq \frac{\eta^2}{\sqrt p} \tau^2 M^2 + \frac{\eta^2}{\sqrt p} \Big( \tau M + \frac{T}{K} \|\theta_*\| \Big) \sum_{i=\tau}^{\frac{T}{K}-1}(1 - \lambda\eta)^{\frac{T}{K}-i-2} \|\theta(i)\|,
    \end{align*}
    where the first inequality follows from $\|\theta(i)\|\leq M$ for all $i\geq 0$ and $\|\theta(i)\|\leq \|\theta_*\|$ for all $\tau\leq i\leq T$. Further, 
    \begin{align*}
        & \frac{\eta^2}{\sqrt p}\sum_{i=T+1}^{t-1}\sum_{j=0}^i\prod_{k=i+1}^{t-1}(1-\tlam(k)) \|\theta(i)\|\|\theta(j)\| \\
        & = \frac{\eta^2}{\sqrt p}\sum_{i=T+1}^{t-1} \|\theta(i)\| \sum_{j=0}^T \|\theta(j)\| + \frac{\eta^2}{\sqrt p}\sum_{i=T+1}^{t-1} \|\theta(i)\| \sum_{j=T}^i\|\theta(j)\| \\
        & \leq \frac{\eta^2}{\sqrt p}\sum_{i=T+1}^{t-1} \|\theta(i)\| \Big( \tau M + T\|\theta_*\| + \sum_{j=T}^i \left( 1-\frac{n\eta}{2d} \right)^{j-T} \|\theta(t)\| \Big) \\
        & \leq \frac{\eta^2}{\sqrt p} \Big( \tau M + T\|\theta_*\| + \frac{2d}{n\eta} \|\theta_*\| \Big) \sum_{i=T+1}^{t-1} \left( 1-\frac{n\eta}{2d} \right)^{i-T-1} \|\theta(t)\| \\
        & \leq \frac{\eta}{\sqrt p} \Big( \tau M + T\|\theta_*\| + \frac{2d}{n\eta} \|\theta_*\| \Big) \frac{2d}{n} \|\theta_*\|,
    \end{align*}
    where the first inequality follows from $\|\theta(i)\|\leq M$ for all $i\geq 0$, $\|\theta(i)\|\leq \|\theta_*\|$ for all $\tau\leq i\leq T$, and $\|\theta(i)\|$ decays exponentially fast at rate $1-\frac{n\eta}{2d}$. The second and third inequalities are due to a sum of geometric series.
    
    On the other hand, 
    \begin{align*}
        & \frac{\eta^2}{\sqrt p}\sum_{i=T+1}^{t-1}\sum_{j=0}^i\prod_{k=i+1}^{t-1}(1-\tlam(k)) \theta(i)\transpose\theta(j) \\
        & = \frac{\eta^2}{\sqrt p}\sum_{i=T+1}^{t-1}\sum_{j=0}^i (a(i) a(j) - \|\xi(i)\|\|\xi(j)\|) \\
        & = \frac{\eta^2}{\sqrt p}\sum_{j=0}^T \sum_{i=T+1}^{t-1} (a(i) a(j) - \|\xi(i)\|\|\xi(j)\|) + \frac{\eta^2}{\sqrt p} \sum_{j=T+1}^{t-1} \sum_{i=j+1}^{t-1} (a(i) a(j) - \|\xi(i)\|\|\xi(j)\|) \\
        & \geq \frac{\eta^2}{\sqrt p}\sum_{j=0}^T \sum_{i=T+1}^{t-1} \theta(i)\transpose\theta(j) - \frac{\eta^2}{\sqrt p} \sum_{j=T+1}^{t-1} \sum_{i=j+1}^{t-1} \|\theta(i)\|\|\theta(j)\|,
    \end{align*}
    where
    \begin{align*}
        \frac{\eta^2}{\sqrt p} \sum_{j=T+1}^{t-1} \sum_{i=j+1}^{t-1} \|\theta(i)\|\|\theta(j)\| & \leq \frac{\eta^2}{\sqrt p} \sum_{j=T+1}^{t-1} \|\theta(j)\| \sum_{i=j+1}^{t-1} \left( 1-\frac{n\eta}{2d} \right)^{i-j-1} \|\theta_{j+1}\| \\
        & \leq \frac{\eta^2}{\sqrt p} \sum_{j=T+1}^{t-1} \left( 1-\frac{n\eta}{2d} \right)^{j-T-1} \|\theta(t+1)\| \frac{2d}{n\eta} \|\theta_*\| \\
        & \leq \frac{4d^2}{n^2\sqrt{p}} \|\theta_*\|^2,
    \end{align*}
    % and 
    % \begin{align*}
    %     \frac{\eta^2}{\sqrt p}\sum_{j=0}^T \sum_{i=T+1}^{t-1} \theta(i)\transpose\theta(j) & \geq \frac{\eta^2}{\sqrt p}\sum_{j=\tau}^T \sum_{i=T+1}^{t-1} \theta(i)\transpose\theta(j) - \frac{\eta^2}{\sqrt p}\sum_{j=0}^{\tau-1} \sum_{i=T+1}^{t-1} \|\theta(i)\|\|\theta(j)\| \\
    %     & \geq \frac{\eta^2}{\sqrt p}\sum_{j=\tau}^T \theta(j)\transpose \sum_{i=T+1}^{t-1} \theta(i) - \frac{\eta^2}{\sqrt p} \tau M \frac{2d}{n\eta} \|\theta_*\|,
    % \end{align*}
    where the second and third inequalities are due to taking the limit of geometric series.
    
    Recall that we define $s(T) = \sum_{j=0}^T \theta(j)$, and we can write $\frac{\eta^2}{\sqrt p}\sum_{j=0}^T \theta(j)\transpose \sum_{i=T+1}^{t-1} \theta(i) = \frac{\eta^2}{\sqrt p} \sum_{i=T+1}^{t-1} s(T)\transpose \theta(i)$. As long as $s(T)\transpose \theta(t)$ is large enough compared to $\|\theta(t)\|$ and further perturbations on $\theta(t)$ quickly fade away for all $t > T$, we can lower bound $\frac{\eta^2}{\sqrt p}\sum_{j=0}^T \theta(j)\transpose \sum_{i=T+1}^{t-1} \theta(i)$ with $\eta C\sum_{i=T}^{t-1} \|\theta(i)\|$ for some $C>0$. In particular, because $a(t) \geq \frac{(\lambda - \frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}}$ and $\|\Xi(t)\| \leq \frac{\frac{n}{d}\|\theta_*\|}{\lambda + \frac{n}{2d}}$ with $\lambda\geq \frac{12n}{d}$, we have $a(t) \geq 2\|\Xi(t)\|$. Let us denote $s(T) = a_{s(T)}\hat\theta_* + \xi_{s(T)}$ using an orthogonal decomposition, where $a_{s(T)}$ is the amount of contribution in the direction of $\theta_*$ and $\xi_{s(T)}$ represents its orthogonal complement. Since $a(t)\leq \|\theta(t)\|$ for any $t\leq \tau$ and $a(t) \geq \frac{(\lambda - \frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}}$ and $\|\Xi(t)\| \leq \frac{\frac{n}{d}\|\theta_*\|}{\lambda + \frac{n}{2d}}$ for any $\tau\leq t\leq T$, it holds
    \begin{align*}
        a_{s(T)} \geq (T-\tau) \frac{(\lambda - \frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} - \tau M, \qquad \|\xi_{s(T)}\| \leq (T-\tau) \frac{\frac{n}{d}\|\theta_*\|}{\lambda + \frac{n}{2d}} + \tau M.
    \end{align*}
    We can also get $a_{s(T)} \geq 2 \|\xi_{s(T)}\|$ if $T \geq 2\tau$ under the condition that $\sqrt{p} \geq 16n\eta\tau/\sqrt{d}$ and 
    \begin{align*}
        \sqrt{p} \geq 96\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\frac{\eta n^2}{d}\tau \frac{\frac{2n}{d}}{\lambda + \frac{n}{2d}}\frac{1}{\|\theta_*\|}.
    \end{align*}
    Let us denote $\alpha(t) \defeq \frac{1}{\sqrt{p}}\theta(t)\transpose s(T)$ for all $t\geq T$, and we have $\alpha(t) = \frac{1}{\sqrt{p}}\theta(t)\transpose s(T) \geq \frac{1}{\sqrt{p}}(a(t) a_{s(T)} - \|\Xi(t)\|\|\xi_{s(T)}\|) \geq \frac{3}{4\sqrt{p}} a(t) a_{s(T)}$, where $a(t) \geq \frac{(\lambda - \frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} \geq \frac{1}{2}\|\theta_*\|$ and 
    \begin{align*}
        \frac{1}{\sqrt{p}} a_{s(T)} & \geq \frac{T-\tau}{\sqrt{p}} \frac{(\lambda - \frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} - \frac{\tau}{\sqrt{p}} M \geq \frac{T}{4\sqrt{p}} \|\theta_*\| - \frac{\tau}{\sqrt{p}} M \geq \frac{\sqrt{d}}{64\eta n} \|\theta_*\|
    \end{align*}
    if $\tau M \leq \frac{T}{8}$ under the condition that $\sqrt{p}\geq 128 \left(1 + \sqrt{8\log(d/\delta)}\right) \frac{n^2\eta\tau}{d}$. Combine them together to get $\alpha(t) \geq \frac{3}{8}\frac{\sqrt{d}}{64\eta n} \|\theta_*\|^2 \geq \frac{3\sqrt{d}}{512n\eta} \|\theta(t)\|^2 \geq \frac{3\sqrt{d}}{512n\eta} \|\theta(t)\|$ \icomment{Require lower bound on $\|\theta_*\|$}.
    
    Remember that for any $t>T$, the update rule on $\theta(t)$ writes
    \begin{align*}
        \theta(t+1) & = \Big( I_d - \frac{n\eta}{d} I_d - \eta\Delta(t) + \frac{\eta}{\sqrt p}\Xi(t)  - (1-\lambda\eta)^{T+1} \frac{\eta}{p} b\transpose\beta(0) \Sigma^2 + \frac{n\eta}{d}I_d - \frac{\eta}{p}\Sigma^2 W(0)\transpose W(0) \Big)\theta(t) \\
        & = \Big( I_d - \frac{n\eta}{d} I_d - \frac{\eta^3}{p^2} \|b\|^2 \Sigma^2 s(T) s(t-1)\transpose \Big)\theta(t) \\
        & \qquad + \Big( \frac{\eta}{\sqrt{p}} \Phi_t + \frac{\eta}{\sqrt p}\Xi(t)  - (1-\lambda\eta)^{T+1} \frac{\eta}{p} b\transpose\beta(0) \Sigma^2 + \frac{n\eta}{d}I_d - \frac{\eta}{p}\Sigma^2 W(0)\transpose W(0) \Big)\theta(t),
    \end{align*}
    where $\Delta(t) = \frac{\eta^2}{p^2} \|b\|^2\big(\sum_{i=0}^t\sum_{j=0}^i \prod_{k=i+1}^T (1-\eta\lambda)\theta(j)\transpose \theta(i) \Sigma^2 + \Sigma^2 s(T) s(t-1)\transpose \big)$, $\Phi_t \defeq \frac{\eta}{p\sqrt{p}} \|b\|^2 \sum_{i=0}^t\sum_{j=0}^i \prod_{k=i+1}^T (1-\eta\lambda)\theta(j)\transpose \theta(i) \Sigma^2$ and $\Xi(t) = \frac{\eta}{\sqrt p}\big(u\transpose \tilde{s}(t) \Sigma^2 + \Sigma^2 u s(t-1)\transpose + \Sigma^2 s(t-1)u\transpose\big)$. Notice that $\frac{1}{p} s(T)\transpose(s(T) s(T)\transpose)\theta(t) = \frac{\|s(T)\|^2}{p} \alpha(t)$, we further split $s(T) = s(T) + (s(T) - s(T))$ to get
    \begin{align*}
        s(T) s(t-1)\transpose = s(T) s(T)\transpose + \underbrace{(s(T) - s(T)) s(t-1)\transpose + s(T) (s(t-1) - s(T))\transpose + (s(T) - s(T))(s(t-1) - s(T))\transpose}_{\Psi(t)},
    \end{align*}
    and we define a shorthand $\Psi(t)$ to represent the remaining tails that are going to be proved as smaller terms. Given the shorthand, we can further rewrite the update rule on $\theta(t)$ into
    \begin{align}
        \begin{split}\label{eqn:update-split}
            \theta(t+1) & = \Big( I_d - \frac{n\eta}{d} I_d - \frac{\eta^3}{p^2} \|b\|^2 \Sigma^2 s(T) s(T)\transpose \Big)\theta(t) \\
            & \qquad + \Big( \frac{\eta}{\sqrt{p}} \Phi_t + \frac{\eta}{\sqrt p}\Xi(t)  - (1-\lambda\eta)^{T+1} \frac{\eta}{p} b\transpose\beta(0) \Sigma^2 + \frac{n\eta}{d}I_d - \frac{\eta}{p}\Sigma^2 W(0)\transpose W(0) - \frac{\eta^3}{p^2} \|b\|^2 \Sigma^2 \Psi(t) \Big)\theta(t).
        \end{split}
    \end{align}
    Multiply $\frac{1}{\sqrt{p}} s(T)\transpose$ on both sides of \cref{eqn:update-split}, we have
    \begin{align*}
        \alpha(t+1) & = \Big( 1 - \frac{n\eta}{d} - \frac{n\eta^3}{dp^2} \|b\|^2 \|s(T)\|^2 \Big) \alpha(t) \\
        & \qquad + \frac{1}{\sqrt{p}} s(T)\transpose \Big( \frac{\eta}{\sqrt{p}} \Phi_t + \frac{\eta}{\sqrt p}\Xi(t)  - (1-\lambda\eta)^{T+1} \frac{\eta}{p} b\transpose\beta(0) \Sigma^2 + \frac{n\eta}{d}I_d - \frac{\eta}{p}\Sigma^2 W(0)\transpose W(0) - \frac{\eta^3}{p^2} \|b\|^2 \Sigma^2 \Psi(t) \\
        & \qquad + \frac{\eta^3}{p^2} \|b\|^2 (\frac{n}{d}I_d - \Sigma^2) s(T) s(T)\transpose \Big)\theta(t) \\
        & \geq \Big( 1 - \frac{n\eta}{d} - \frac{n\eta^3}{dp^2} \|b\|^2 \|s(T)\|^2 \Big) \alpha(t) \\
        & \qquad - \frac{1}{\sqrt{p}} \|s(T)\|\|\theta(t)\| \Big( \frac{\eta}{\sqrt{p}} \|\Phi_t\| + \frac{\eta}{\sqrt p} \|\Xi(t)\| + (1-\lambda\eta)^{T+1} \frac{\eta}{p} |b\transpose\beta(0)| \|\Sigma^2\| + \Big\| \frac{n\eta}{d}I_d - \frac{\eta}{p}\Sigma^2 W(0)\transpose W(0) \Big\| \\
        & \qquad + \frac{\eta^3}{p^2} \|b\|^2 \|\Sigma^2\| \|\Psi(t)\| + \frac{\eta^3}{p^2} \|b\|^2 \|s(T)\|^2 \Big\| \frac{n}{d}I_d - \Sigma^2 \Big\| \Big).
    \end{align*}
    In particular, if $p \geq 16\log\frac{2}{\delta}$ and $\tau M \leq (T-\tau) \|\theta_*\|$ under the condition that
    \begin{align*}
        \sqrt{p} \geq \left( \tau + \left(1 + \sqrt{8\log\frac{2d}{\delta}}\right) \right) \frac{8n\eta}{\sqrt{d}},
    \end{align*}
    we have
    \begin{align*}
        \frac{n\eta^3}{dp^2} \|b\|^2 \|s(T)\|^2 & \leq (1 + 4\sqrt{\log(1/2\delta)/p}) \frac{n\eta^3}{dp} (\tau M + (T-\tau) \|\theta_*\|)^2 \\
        & \leq (1 + 4\sqrt{\log(1/2\delta)/p}) \frac{4n\eta^3}{dp} T^2 \|\theta_*\|^2 \\
        & \leq (1 + 4\sqrt{\log(1/2\delta)/p}) \frac{\eta}{4n} \|\theta_*\|^2 \\
        & \leq \frac{\eta}{2n} \|\theta_*\|^2 \\
        & \leq \frac{(1+\eps)n}{2d}\eta,
    \end{align*}
    where the first inequality is due to \cref{cor:b-norm-concentration} and triangular inequality, the second inequality is due to $\tau M \leq (T-\tau) \|\theta_*\|$, the third inequality follows from $T \leq \frac{\sqrt{d}}{4\eta n}\sqrt{p}$, the fourth inequality follows from $p \geq 16\log\frac{2}{\delta}$, and the last inequality follows from $\|\theta_*\| \leq \|X\|\|y\|$.
    
    Note that $\frac{1}{\sqrt{p}} \|s(T)\|\leq \frac{2T}{\sqrt{p}} \|\theta_*\| \leq \frac{\sqrt{d}}{2n\eta} \|\theta_*\| \leq \frac{1+\eps}{2\eta}$ for $\tau M \leq (T-\tau) \|\theta_*\|$, and if $\sqrt{p}\geq 96(1+\eps)^2 d\sqrt{8\log(d/\delta)}(1 + \sqrt{8\log(d/\delta)})$, then with probability at least $1-5\delta$ that
    \begin{align*}
        \|\Xi(t)\| & \leq \frac{3(1+\eps)n\eta}{d\sqrt{p}} \|u\|\|s(T)\| \leq \frac{n}{8d},
    \end{align*}
    \begin{align*}
        \frac{1}{\sqrt{p}}|b\transpose\beta(0)| \|\Sigma^2\| & \leq \frac{(1+\eps)n}{d}\sqrt{8\log\frac{2}{\delta}} \leq (1+\eps)\sqrt{8\log\frac{2}{\delta}} \cdot \frac{n}{d},
    \end{align*}
    and
    \begin{align*}
        \Big\| \frac{1}{p}\Sigma^2 W(0)\transpose W(0) - \frac{n}{d} I_d \Big\| \leq \frac{\eps n}{d}.
    \end{align*}
    Further, we also have upper bounds:
    \begin{align*}
        \frac{\eta^3}{p^2} \|b\|^2 \|s(T)\|^2 \Big\| \frac{n}{d}I_d - \Sigma^2 \Big\| & \leq \left(1 + \frac{4}{\sqrt p}\sqrt{\log\frac{2}{\delta}}\right) \frac{\eta^3}{p}\cdot 4T^2 \|\theta_*\|^2 \frac{\eps n}{d} \\
        & \leq \left(1 + \frac{4}{\sqrt p}\sqrt{\log\frac{2}{\delta}}\right) \frac{\eps\eta}{4n} \|\theta_*\|^2 \\
        & \leq (1+\eps) \left(1 + \frac{4}{\sqrt p}\sqrt{\log\frac{2}{\delta}}\right) \frac{\eps\eta}{4n}\frac{n^2}{d} \\
        & \leq \frac{\eps\eta n}{d}
    \end{align*}
    if $p \geq 16\log\frac{2}{\delta}$, and
    \begin{align*}
        \frac{\eta^3}{p^2} \|b\|^2 \|\Sigma^2\| \|\Psi(t)\| & \leq (1+\eps) \left(1 + \frac{4}{\sqrt p}\sqrt{\log\frac{2}{\delta}}\right) \frac{\eta^3}{p} \frac{n}{d} \|\Psi(t)\|,
    \end{align*}
    where 
    \begin{align*}
        \|\Psi(t)\| & \leq \|s(T) - s(T)\| \|s(t-1)\| + \|s(T)\| \|s(t-1) - s(T)\| + \|s(T) - s(T)\|\|s(t-1) - s(T)\| \\
        & \leq 2\sum_{i=T}^t \|\theta(i)\| \Big( \sum_{i=0}^T \|\theta(i)\| + \sum_{i=T}^t \|\theta(i)\| \Big) + \Big( \sum_{i=T}^t \|\theta(i)\| \Big)^2 \\
        & \leq \sum_{i=T}^t \|\theta(i)\| \sum_{i=0}^T \|\theta(i)\| + 3\Big( \sum_{i=T}^t \|\theta(i)\| \Big)^2,
    \end{align*}
    and from previous arguments we have $\sum_{i=0}^T \|\theta(i)\| \leq \tau M + (T-\tau) \|\theta_*\| \leq 2T \|\theta_*\|$ and $\sum_{i=T}^t \|\theta(i)\| \leq \frac{2d}{n\eta}\|\theta_*\|$. Combine them to get 
    \begin{align*}
        \frac{\eta^3}{p^2} \|b\|^2 \|\Sigma^2\| \|\Psi(t)\| & \leq (1+\eps) \left(1 + \frac{4}{\sqrt p}\sqrt{\log\frac{2}{\delta}}\right) \frac{\eta^3}{p} \frac{n}{d} \frac{6d}{n\eta} T \|\theta_*\|^2 \\
        & \leq (1+\eps) \left(1 + \frac{4}{\sqrt p}\sqrt{\log\frac{2}{\delta}}\right) \frac{3\eta}{\sqrt{p}} \frac{\sqrt{d}}{2n} \|\theta_*\|^2 \\
        & \leq (1+\eps)^2 \left(1 + \frac{4}{\sqrt p}\sqrt{\log\frac{2}{\delta}}\right) \frac{3\eta}{\sqrt{p}} \frac{n}{2\sqrt{d}} \\
        & \leq \frac{12n\eta}{\sqrt{dp}}.
    \end{align*}
    Finally, we have 
    \begin{align*}
        \|\Phi_t\| & \leq \frac{\eta}{p\sqrt{p}} \|b\|^2 \|\Sigma^2\| \Big( \sum_{i=0}^{T-1} (1-\eta\lambda)^{T-i-1}\theta(i)\transpose  \sum_{j=0}^i \theta(j) + \sum_{i=T}^t \theta(i)\transpose  \sum_{j=0}^i \theta(j) \Big) \\
        & \leq \frac{\eta}{p\sqrt{p}} \|b\|^2 \|\Sigma^2\| \Big[ \sum_{i=0}^{T-1} (1-\eta\lambda)^{T-i-1} \|\theta(i)\|  \sum_{j=0}^{T-1} \|\theta(j)\| + \sum_{i=T}^t \|\theta(i)\|  \Big( \sum_{j=0}^{T-1} \|\theta(j)\| + \sum_{j=T}^i \|\theta(j)\| \Big) \Big] \\
        & \leq \frac{\eta(1+\eps)n}{d\sqrt{p}} \left(1 + \frac{4}{\sqrt p}\sqrt{\log\frac{2}{\delta}}\right) \Big[ \Big( \tau M + \frac{1}{\lambda\eta} \|\theta_*\| \Big) 2T \|\theta_*\| + \frac{2d}{n\eta}\|\theta_*\|  \Big( 2T \|\theta_*\| + \frac{2d}{n\eta}\|\theta_*\| \Big) \Big] \\
        & \leq \frac{4\eta n}{d\sqrt{p}} \left[ (1+\eps)^2 (1+\eps)\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right) \tau \frac{n\sqrt{p}}{2\eta d} + (1+\eps) \frac{n\sqrt{p}}{2\lambda\eta^2\sqrt{d}} + (1+\eps) \frac{\sqrt{p}}{\eta^2\sqrt{d}} + \frac{4d}{\eta^2} \right] \\
        & \leq 8\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right) \tau \frac{2n^2}{d^2} + \frac{2n^2}{\lambda\eta d\sqrt{d}} + \frac{8n}{\eta d\sqrt{d}} + \frac{16n}{\eta\sqrt{p}} \\
        & \leq 8\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right) \tau \frac{2n^2}{d^2} + \frac{n}{6\eta \sqrt{d}} + \frac{8n}{\eta d\sqrt{d}} + \frac{16n}{\eta\sqrt{p}}.
    \end{align*}
    Hence, all the small terms can be bounded by
    \begin{align*}
        &\frac{1}{\sqrt{p}} \|s(T)\|\|\theta(t)\| \Big( \frac{\eta}{\sqrt{p}} \|\Phi_t\| + \frac{\eta}{\sqrt p} \|\Xi(t)\| + (1-\lambda\eta)^{T+1} \frac{\eta}{p} |b\transpose\beta(0)| \|\Sigma^2\| + \Big\| \frac{n\eta}{d}I_d - \frac{\eta}{p}\Sigma^2 W(0)\transpose W(0) \Big\| \\
        & \qquad + \frac{\eta^3}{p^2} \|b\|^2 \|\Sigma^2\| \|\Psi(t)\| + \frac{\eta^3}{p^2} \|b\|^2 \|s(T)\|^2 \Big\| \frac{n}{d}I_d - \Sigma^2 \Big\| \Big) \\
        & \leq \frac{1+\eps}{2\eta}  \Big[ \frac{\eta}{\sqrt{p}} \Big( 8\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right) \tau \frac{2n^2}{d^2} + \frac{n}{6\eta \sqrt{d}} + \frac{8n}{\eta d\sqrt{d}} + \frac{16n}{\eta\sqrt{p}} \Big) + \frac{\eta}{\sqrt p} \frac{n}{8d} \\
        & \qquad + (1+\eps)\sqrt{8\log\frac{2}{\delta}} \cdot \frac{n}{d\sqrt{p}} + \frac{\eps n\eta}{d} + \frac{12n\eta}{\sqrt{dp}} + \frac{\eps\eta n}{d} \Big] \|\theta(t)\| \\
        & \leq \Big[ \frac{1}{\sqrt{p}} \Big( 8\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right) \tau \frac{2n^2}{d^2} + \frac{n}{6\eta \sqrt{d}} + \frac{8n}{\eta d\sqrt{d}} + \frac{16n}{\eta\sqrt{p}} \Big) + \frac{n}{8d\sqrt{p}} \\
        & \qquad + 2\sqrt{8\log\frac{2}{\delta}} \cdot \frac{n}{\eta d\sqrt{p}} + \frac{2\eps n}{d} + \frac{12n}{\sqrt{dp}} \Big] \|\theta(t)\|
    \end{align*}
    
    Consequently, we have $\alpha(t+1) \geq (1-2\frac{n\eta}{d})\alpha(t) + \frac{3\eps n}{d}\|\theta(t)\|$ when $p\geq \icomment{TODO}$ and for all $t>T$ it holds
    \begin{align*}
        \alpha(t) \geq \Big( 1-\frac{2n\eta}{d} \Big)^{t-T}\alpha(t) - \frac{3\eps n}{d} \sum_{i=0}^{t-T} \Big( 1-\frac{2n\eta}{d} \Big)^{t-T-i} \|\theta(i)\|.
    \end{align*}
    Summing over all $t>T$ to get
    \begin{align*}
        \sum_{t=T}^\infty\alpha(t) & \geq \sum_{t=T}^\infty \Big( 1-\frac{2n\eta}{d} \Big)^{t-T}\alpha(t) - \sum_{t=T}^\infty \frac{3\eps n}{d} \sum_{i=0}^{t-T} \Big( 1-\frac{2n\eta}{d} \Big)^{t-T-i}\|\theta(i)\| \\
        & \geq \frac{d}{2n\eta}\alpha(t) - \frac{3\eps n}{d} \sum_{t=T}^\infty\sum_{i=0}^{t-T} \Big( 1-\frac{2n\eta}{d} \Big)^{t-T-i}\|\theta(i)\| \\
        &\geq \frac{d}{2n\eta}\alpha(t) - \frac{3\eps n}{d} \sum_{i=0}^\infty\|\theta_{i+T}\|\sum_{t=T}^\infty \Big( 1-\frac{2n\eta}{d} \Big)^{t-T-i} \\
        &\geq \frac{d}{2n\eta}\alpha(t) - \frac{\frac{3\eps n}{d} d}{2n\eta} \sum_{i=0}^\infty \Big( 1-\frac{n\eta}{2d} \Big)^i \|\theta_{T}\| \\
        &\geq \frac{d}{2n\eta} \frac{3\sqrt{d}}{512n\eta^2} \|\theta(t)\|^2 - \frac{\frac{3\eps n}{d} d^2}{n^2\eta} \|\theta(t)\| \\
        &\geq \frac{3d\sqrt{d}}{1024n^2\eta^3} \|\theta(t)\|^2 - \frac{d^2}{n^2\eta^2} \frac{3\eps n}{d} \|\theta(t)\| \\
        &\geq \frac{3d\sqrt{d}}{2048n^2\eta^3} \|\theta_*\| \|\theta(t)\| - \frac{d^2}{n^2\eta^2} \frac{3\eps n}{d} \|\theta(t)\| \icomment{Require lower bound on $\|\theta_*\|$} \\
        & \geq \Big( \frac{3}{2048\eta} - 3\eps \Big) \frac{d}{n\eta^2} \|\theta(t)\|.
    \end{align*}
    This implies that $\frac{\eta^2}{\sqrt p}\sum_{j=0}^T \theta(j)\transpose \sum_{i=T+1}^{t-1} \theta(i) = \frac{\eta^2}{\sqrt p} \sum_{i=T+1}^{t-1} s(T)\transpose \theta(i) = \eta^2 \sum_{t=T}^\infty\alpha(t) \geq ( \frac{3}{2048\eta} - 3\eps ) \frac{d}{n} \|\theta(t)\|$. Recall that $\eta\sum_{i=T}^{t-1} \|\theta(i)\| \leq \frac{2d}{n} \|\theta(t)\|$. For any $\eps\eta \leq \frac{1}{2\times 6144}$, we have
    \begin{align*}
        \frac{\eta^2}{\sqrt p}\sum_{j=0}^T \theta(j)\transpose \sum_{i=T+1}^{t-1} \theta(i) \geq \frac{\frac{3}{2048\eta} - 3\eps}{2} \cdot \eta\sum_{i=T}^{t-1} \|\theta(i)\|.
    \end{align*}
    
    % In particular, the first term can be upper bounded with
    % \begin{align*}
    %     \eta\sum_{i=\tau}^{T-1} (1-\lambda\eta)^{T-i-2}\|\theta(i)\| & \leq \frac{\eta^2}{2\sqrt p}\sum_{i=\tau}^{T-1}\prod_{k=i+1}^{t-1}(1-\tlam(k))a(i)\sum_{j=0}^{i-1} a(j) \leq C_5\|\phi_{3}(t)\|, \icomment{TODO}
    % \end{align*}
    % where $\|\phi_{2}(t)\| \gtrsim \eta\sum_{i=0}^{t-1}(1-\lambda\eta)^i \simeq \frac{1}{\lambda}$.
    
    % Recall that $a_0 \geq -\|\theta(0)\|\geq -(1+\eps)(1 + \sqrt{8\log\frac{2d}{\delta}})\frac{n}{\sqrt{d}}$ with probability at least $1-3\delta$, and for any initialization starting $a_0\leq \frac{(\lambda - \frac{n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}}$, it converges to the quantity exponentially fast. More specifically, for any $\lambda\geq \frac{4n}{d}$, we have with probability at least $1-3\delta$ that
    % \begin{align*}
    %     (1-\eps)\frac{n}{\sqrt{d}} \leq \|\theta_*\| \leq (1+\eps)\frac{n}{\sqrt{d}}.
    % \end{align*}
    % Let us denote $\tau_0$ be the first time that $a(t)\geq 0$, then it holds that 
    % \begin{align*}
    %     \tau_0 & \leq \log\left[ \frac{\lambda+\frac{2n}{d}}{(\lambda-\frac{n}{d})\|\theta_*\|} \left( \frac{(\lambda - \frac{n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} + (1+\eps)\Big( 1 + \sqrt{8\log\frac{2d}{\delta}} \Big)\frac{n}{\sqrt{d}} \right) \right]/\log\frac{1}{1 - (\lambda+\frac{n}{2d})\eta} \\
    %     & \leq \log \left( 1 + \frac{2(1+\eps)}{1-\eps} \Big( 1 + \sqrt{8\log\frac{2d}{\delta}} \Big) \right) / \log\frac{1}{1 - (\lambda+\frac{n}{2d})\eta}.
    % \end{align*}
    % Therefore, we have $\sum_{j=0}^{\tau_0-1} |a(j)| \leq \tau_0\|\theta(0)\| \leq (1+\eps)(1 + \sqrt{8\log\frac{2d}{\delta}})\frac{n\tau_0}{\sqrt{d}}$. Recall that for any $t$ falls between $\tau$ and $T$, it holds that $a(t)\geq \frac{(\lambda - \frac{2n}{d})\|\theta_*\|}{\lambda + \frac{2n}{d}} \geq \frac{1}{3}\|\theta_*\| \geq \frac{1}{3}(1-\eps)\frac{n}{\sqrt{d}}$. Consequently, we have $\sum_{j=0}^t a(j) \geq 0$ for any $t\geq \tau' = \tau+\bar\tau$, where
    % \begin{align*}
    %     \bar\tau = \frac{3(1+\eps)}{1-\eps} \Big( 1 + \sqrt{8\log\frac{2d}{\delta}} \Big) \tau_0.
    % \end{align*}
    % As long as $\tau'\leq\frac{T}{4}$\icomment{TODO: calculate conditions on $p$}, the first term can be further bounded by
    % \begin{align*}
    %     \frac{\eta^2}{2\sqrt p} \sum_{i=\frac{T}{K}}^{T-1} (1-\lambda\eta)^{t-i-2} |a(i)| \cdot \Big( \sum_{j=0}^{\tau'-1} a(j) + \sum_{j=\tau'}^{i-1} a(j) \Big) & \geq \frac{\eta^2}{2\sqrt p} \sum_{i=\frac{T}{K}}^{T-1} (1-\lambda\eta)^{t-i-2} |a(i)| \cdot \frac{T}{4} \cdot \frac{1}{3}(1-\eps)\frac{n}{\sqrt{d}} \\
    %     & \geq \frac{\eta}{48}(1-\eps) \sum_{i=\frac{T}{K}}^{T-1} (1-\lambda\eta)^{t-i-2} |a(i)|,
    % \end{align*}
    % where the first inequality follows from $\tau'\leq \frac{T}{4}$ and $a(t)\geq \frac{1}{3}(1-\eps)\frac{n}{\sqrt{d}}$ for $t\geq\tau'$ and the second inequality follows from $T \geq \frac{\sqrt{d}}{8\eta n}\sqrt{p}$.
    
    Putting the pieces together, we have
    \begin{align*}
        \|\phi_{2}(t)\| & \leq  \eta\sum_{i=\frac{T}{K}}^{T-1} (1-\lambda\eta)^{T-i-2} \|\theta(i)\| + \eta\sum_{i=0}^{\frac{T}{K}-1}\prod_{k=i+1}^{\frac{T}{K}-1}(1-\tlam(k)) \|\theta(i)\| + \eta\sum_{i=T}^{t-1} \prod_{k=T+1}^{t-1}(1-\tlam(k)) \|\theta(i)\| \\
        & \leq \eta\sum_{i=\frac{T}{K}}^{T-1} (1-\lambda\eta)^{T-i-2} \|\theta(i)\| + \frac{2d}{n} \|\theta(t)\| + \eta\tau M + \frac{1}{\lambda} \|\theta_*\| 
    \end{align*}
    and 
    \begin{align*}
        \|\phi_{3}(t)\| 
        & \geq \frac{\eta^2}{\sqrt p}\sum_{i=\frac{T}{K}}^{T}\prod_{k=i+1}^{T-1}(1-\lambda\eta)\theta(i)\transpose\sum_{j=0}^{i-1} \theta(j) - \frac{\eta^2}{\sqrt p}\sum_{i=0}^{\frac{T}{K}-1}\sum_{j=0}^i\prod_{k=i+1}^{\frac{T}{K}-1}(1-\tlam(k)) \|\theta(i)\|\|\theta(j)\| \\
        & \qquad + \frac{\eta^2}{\sqrt p}\sum_{i=T+1}^{t-1}\sum_{j=0}^i\prod_{k=i+1}^{t-1}(1-\tlam(k)) \theta(i)\transpose \theta(j) \\
        & \geq \frac{\sqrt{5}(1-\eps)}{560} \cdot \eta\sum_{i=\frac{T}{K}}^{T-1}(1-\lambda\eta)^{T-i-2} \|\theta(i)\| + \Big( \frac{3}{2048\eta} - 3\eps \Big) \frac{d}{n} \|\theta(t)\| \\
        & \qquad - \frac{\eta^2}{\sqrt p} \tau^2 M^2 - \frac{\eta^2}{\sqrt p} \Big( \tau M + \frac{T}{K} \|\theta_*\| \Big) \sum_{i=\tau}^{\frac{T}{K}-1}(1 - \lambda\eta)^{\frac{T}{K}-i-2} \|\theta(i)\|.
    \end{align*}
    Let us define $A(T,K) \defeq \eta\sum_{i=\frac{T}{K}}^{T-1}(1-\lambda\eta)^{T-i-2} \|\theta(i)\|$ and $B(T) \defeq \frac{d}{n} \|\theta(t)\|$, and we can we can rewrite the above inequalities into
    \begin{align*}
        \|\phi_{2}(t)\| & \leq A(T,K) + 2B(T) + \eta\tau M + \frac{1}{\lambda} \|\theta_*\|
    \end{align*}
    and
    \begin{align*}
        \|\phi_{3}(t)\| & \geq \frac{\sqrt{5}}{1120} A(T,K) + \frac{3}{4096\eta} B(T) - \frac{\eta^2}{\sqrt p} \tau^2 M^2 - \frac{\eta^2}{\sqrt p} \Big( \tau M + \frac{T}{K} \|\theta_*\| \Big) \sum_{i=\tau}^{\frac{T}{K}-1}(1 - \lambda\eta)^{\frac{T}{K}-i-2} \|\theta(i)\|.
    \end{align*}
    Note that $B(T) \geq \frac{d}{2n} \|\theta_*\|$ and
    \begin{align*}
        A(T,K) & \geq \eta\sum_{i=\frac{T}{K}}^{T-1}(1-\lambda\eta)^{T-i-2} |a(i)| \geq \frac{\eta}{2}\sum_{i=\frac{T}{K}}^{T-1}(1-\lambda\eta)^{T-i-2} \|\theta_*\| \geq \frac{\eta}{2} \frac{1 - (\lambda\eta)^{(1-1/K)T}}{\lambda\eta} \|\theta_*\| \geq \frac{1}{4\lambda} \|\theta_*\|,
    \end{align*}
    where the last inequality follows from the condition that $\sqrt{p} \geq 2 \frac{\log 2}{\log\frac{d}{12n\eta}}\frac{8n\eta}{\sqrt{d}}$. Hence, we have 
    \begin{align*}
        \|\phi_{2}(t)\| \leq A(T,K) + \left[ 3 + 8\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\tau \right] B(T),
    \end{align*}
    which is due to $\eps\leq \frac{1}{2}$, $\lambda \geq \frac{12n}{d}$, $M \leq (1+\eps)\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\frac{n}{\sqrt{d}}$, and $\|\theta_*\|\geq (1-\eps)\frac{n}{\sqrt{d}}$ \icomment{Require lower bound on $\|\theta_*\|$}. Further, we have $\frac{\eta^2}{\sqrt p} \tau^2 M^2 \leq \frac{1}{4096\eta} B(T)$ under the condition that $\sqrt{p} \geq 2\times 8192\eta^3\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)^2 \tau^2 \frac{n^2}{d\sqrt{d}}$. Note that $\sum_{i=\tau}^{\frac{T}{K}-1}(1 - \lambda\eta)^{\frac{T}{K}-i-2} \|\theta(i)\| \leq \sum_{i=\tau}^{\frac{T}{K}-1}(1 - \lambda\eta)^{\frac{T}{K}-i-2} \|\theta_*\| \leq \frac{1}{\lambda\eta} \|\theta_*\|$. We thus have 
    \begin{align*}
        \frac{\eta^2}{\sqrt p} \Big( \tau M + \frac{T}{K} \|\theta_*\| \Big) \sum_{i=\tau}^{\frac{T}{K}-1}(1 - \lambda\eta)^{\frac{T}{K}-i-2} \|\theta(i)\| & \leq \frac{\eta}{\sqrt p} \frac{1}{\lambda} \tau M \|\theta_*\| + \frac{\eta}{\sqrt p} \frac{1}{\lambda} \frac{T}{K} \|\theta_*\| \|\theta_*\| \\
        & \leq \frac{n\eta}{3\sqrt{p}} \left(1 + \sqrt{8\log\frac{2d}{\delta}}\right) \tau + \frac{\sqrt{d}}{48K}.
    \end{align*}
    Recall that with probability at least $1-\delta$ that $B(T) \geq \frac{d}{2n}\|\theta_*\| \geq (1-\eps)\frac{\sqrt{d}}{2}$, and $\frac{\sqrt{d}}{48K} \leq \frac{B(T)}{4096\eta}$ for any $K \geq \frac{1024\eta}{3}$. Similarly, we have $\frac{n\eta}{3\sqrt{p}} \left(1 + \sqrt{8\log\frac{2d}{\delta}}\right) \tau \leq \frac{B(T)}{8192\eta}$ for any $\sqrt{p} \geq \frac{32768n\eta^2}{3\sqrt{d}}\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\tau$.
    Combine the above arguments together, we have 
    \begin{align*}
        \|\phi_{3}(t)\| \geq \frac{\sqrt{5}}{1120} A(T,K) + \frac{1}{8192\eta} B(T).
    \end{align*}
    
    Recall that the cosine value between $b$ and $\beta(t)$ writes
    \begin{align*}
        \cos\angle(b, \beta(t)) & \geq \frac{(1-\eps)\|\phi_{3}(t)\|-\frac{1}{(1-\eps)\sqrt{p}} \sqrt{8d\log\frac{2d}{\delta}} \|\phi_{2}(t)\| - \|\phi_{1}(t)\|}{\|\phi_{1}(t)\|+(1+\eps)\|\phi_{2}(t)\|+(1+\eps)\|\phi_{3}(t)\|} \\
        & \geq \frac{\frac{1}{2}\|\phi_{3}(t)\|-\frac{2}{\sqrt{p}} \sqrt{8d\log\frac{2d}{\delta}} \max\left\{ \frac{1120}{\sqrt{5}}, \frac{1}{8192\eta} \left[ 3 + 8\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\tau \right] \right\} \|\phi_{3}(t)\| - \|\phi_{1}(t)\|}{\|\phi_{1}(t)\|+2\max\left\{ \frac{1120}{\sqrt{5}}, \frac{1}{8192\eta} \left[ 3 + 8\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\tau \right] \right\} \|\phi_{3}(t)\| + 2\|\phi_{3}(t)\|} \\
        & \geq \frac{1}{12 + 8 \max\left\{ \frac{1120}{\sqrt{5}}, \frac{1}{8192\eta} \left[ 3 + 8\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\tau \right] \right\}},
    \end{align*}
    where the second inequality follows from 
    \begin{align*}
        \|\phi_{2}(t)\| \leq \max\left\{ \frac{1120}{\sqrt{5}}, \frac{1}{8192\eta} \left[ 3 + 8\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\tau \right] \right\} \|\phi_{3}(t)\|
    \end{align*}
    and the last inequality follows from $\|\phi_{1}(t)\| \leq \|\phi_{3}(t)\|$ if $\sqrt{p} \geq \frac{2\sqrt{d}}{3}\log\frac{262144}{3\sqrt{d}}$ and the condition that
    \begin{align*}
        \sqrt{p} \geq \max\left\{ \frac{17920}{\sqrt{5}}\sqrt{8\log\frac{2d}{\delta}}, \frac{1}{512\eta} \sqrt{8\log\frac{2d}{\delta}} \left[ 3 + 8\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\tau \right] \right\}.
    \end{align*}
    
    Therefore, we conclude $\cos\angle(b, \beta(t)) = \Theta(1)$.
\end{proof}

\section{Technical Lemmata}

In this section, we present some of the technical lemmata that will be used in proofs.
We will first introduce a variant of the Restricted Isometry Property that bounds the spectral norm of a random Gaussian matrix towards $1$ with high probability.

\begin{lemma}[\citealp{hand2018global}]\label{lem:RIP}
    Let $X\in \Rnd$ has \iid $\calN(0,1/n)$ entries. Fix $0<\varepsilon<1$, $k < n$, and a subspace $T\subseteq \R^d$ of dimension $k$, then there exists universal constants $C$ and $\gamma$, such that with probability at least $1-(C/\varepsilon)^k e^{-\gamma\varepsilon n}$,
    \begin{align*}
    (1-\varepsilon)\|v\|^2_2 \leq \|Xv\|^2_2 \leq (1+\varepsilon)\|v\|^2_2, \quad \forall v\in T.
    \end{align*}
\end{lemma}
Let us take $k = d$ in \cref{lem:RIP} to get the following corollary for the design matrix $X$ with \iid $\calN(0,1/d)$ entries:
\begin{corollary}\label{cor:RIP}
    Let $X\in \Rnd$ has \iid $\calN(0,1/d)$ entries. For any $0<\varepsilon<1$, there exists universal constants $C$ and $\gamma$, such that with probability at least $1-(C/\varepsilon)^d e^{-\gamma\varepsilon n}$,
    \begin{align*}
        (1-\varepsilon)\frac{n}{d}\|v\|^2_2 \leq \|Xv\|^2_2 \leq (1+\varepsilon)\frac{n}{d}\|v\|^2_2, \quad \forall v\in\Rd.
    \end{align*}
    Further, if $\eps \leq C$ and $n \geq \frac{1}{\eps\gamma} (d\log\frac{C}{\eps} + \log\frac{1}{\delta})$, then it holds $\|X\transpose X - \frac{n}{d} I_d\| \leq \frac{n}{d}\varepsilon$ with probability at least $1-\delta$.
\end{corollary}
From \cref{cor:RIP} we have high probability control over the spectral norm of $X\transpose X$ as long as the number of samples $n$ is large enough compared to their dimension $d$.
Similarly, we have the following corollary on $W(0)$ that controls the spectral norm of $X\transpose XW(0)\transpose W(0)$.

\begin{corollary}\label{cor:W0-tail}
    Let $X\in \Rnd$ has \iid $\calN(0,1/d)$ entries and $W(0)\in \Rpd$ has \iid $\calN(0,1)$ entries. For any $0<\varepsilon<1$, there exists universal constants $C$ and $\gamma$, such that if $\eps \leq C$, $n \geq \frac{1}{\eps\gamma} (d\log\frac{C}{\eps} + \log\frac{1}{\delta})$, and $p \geq \frac{1}{\eps\gamma} (d\log\frac{C}{\eps} + \log\frac{1}{\delta})$, then it holds $\|\frac{d}{np}X\transpose XW(0)\transpose W(0) - I_d\| \leq \varepsilon$ with probability at least $1-\delta$.
\end{corollary}

For $\chi^2$ random variables, there are famous tail bounds available.
\begin{lemma}[\citealp{laurent2000adaptive}]\label{lem:chi-squared-tail}
    Suppose $X\sim \chi^2_p$, then for all $t\geq 0$ it holds
    \begin{align*}
        \prob\{X-p \geq 2\sqrt{pt} + 2t\} \leq e^{-t}
    \end{align*}
    and
    \begin{align*}
        \prob\{X-p \leq -2\sqrt{pt}\} \leq e^{-t}.
    \end{align*}
\end{lemma}
For both $b$ and $\beta(0)$ as random Gaussian vectors of dimension $p$, we have $\|b\|^2$ and $\|\beta(0)\|^2$ distributed as independent $\chi^2_p$ random variables, and thus follows the next corollary.
\begin{corollary}\label{cor:b-norm-concentration}
    Suppose $b$ is a random Gaussian vector with independent entries $b_r\sim\calN(0,1)$ for all $r\in[p]$, then for any $p \geq \log\frac{2}{\delta}$, with probability at least $1-\delta$, 
    \begin{align*}
        1 - 2\sqrt{\frac{\log\frac{2}{\delta}}{p}} \leq \frac{\|b\|^2}{p} \leq 1 + 4\sqrt{\frac{\log\frac{2}{\delta}}{p}}.
    \end{align*}
    Further, for $p \geq \frac{16}{\eps^2}\log\frac{2}{\delta}$, it holds $1-\eps \leq \frac{\|b\|^2}{p} \leq 1+\eps$ with probability at least $1-\delta$.
\end{corollary}
In particular, the product of any sub-Gaussian random variables is distributed as a sub-exponential random variable, and the composition property of \iid sub-exponential random variables is illustrated by the following proposition.
\begin{proposition}[\citealp{boucheron2013concentration}]\label{prop:subexponential}
    Suppose $X_i,\ldots,X_p$ are \iid centered sub-exponential random variables with parameter $\nu$ and $\alpha$ such that 
    \begin{align*}
        \expect e^{\lambda X_i} \leq e^{\lambda^2\nu^2/2}
    \end{align*}
    for any $\lambda$ with $|\lambda|<\frac{1}{\alpha}$, then denote it holds
    \begin{align*}
        \prob\bigg( \frac{1}{p}\Big|\sum_{i=1}^p X_i\Big| \geq t \bigg) \leq \exp\bigg( -\frac{p}{2}\min\Big\{ \frac{t^2}{p\nu^2}, \frac{t}{\alpha} \Big\} \bigg).
    \end{align*}
\end{proposition}
% Next, we will introduce Bernstein's inequality \citep{boucheron2013concentration} that may turn out to be useful in later sections.
% \begin{theorem}\label{thm:bernstein}
%     Let $X_1,\ldots,X_p$ be real-valued random variables. Assume that there exist positive numbers $v$ and $c$, such that $\sum_{i=1}^p \expect[X_i^2] \leq v$ and 
%     \begin{align*}
%         \sum_{i=1}^p \expect[(X_i)_+^k] \leq \frac{k!}{2} vc^{k-2}, \qquad k \geq 3.
%     \end{align*}
%     If $S = \sum_{i=1}^p (X_i - \expect[X_i])$, then for all $t \geq 0$, 
%     \begin{align*}
%         \prob\{ S \geq \sqrt{2vt} + ct\} \leq e^{-t}.
%     \end{align*}
% \end{theorem}

% \begin{theorem}\label{thm:inner-product-tail}
%     Let $X,Y\in\Rp$ be independent random Gaussian vectors where $X_r\sim\calN(0,1)$ and $Y_r\sim\calN(0,1)$ independently for all $r\in[p]$, then with probability at least $1-\delta$ that
%     \begin{align*}
%         |\inner{X}{Y}| \leq 4\sqrt{p\log\frac{2}{\delta}}.
%     \end{align*}
% \end{theorem}

% \begin{proof}
%     Due to rotational invariant of random Gaussian vectors, we assume $X$ aligns with the first basis vector, \ie, $X = \|X\|\cdot[1,0,\ldots,0]\transpose$. Hence, we write 
%     \begin{align*}
%         |\inner{X}{Y}| = |Y_1|\cdot\|X\|,
%     \end{align*}
%     where $Y_1$ denotes the first entry of $Y$, which is distributed as $\calN(0,1)$, independent of $X$. From \cref{cor:b-norm-concentration} we know that if $\eps\leq 1$ and $p \geq \frac{16}{\eps^2}\log\frac{2}{\delta}$, it holds $\|b\|\leq (1+\eps)\sqrt{p}\leq 2\sqrt{p}$ with probability at least $1-\frac{\delta}{2}$. Recall that for Gaussian random variable $Y_1\sim\calN(0,1)$, we have $\prob\{|Y_1|\geq t\}\leq 2e^{-t^2/2}$, \ie, $|Y_1| \leq 2\sqrt{\log\frac{2}{\delta}}$ with probability at least $1-\frac{\delta}{2}$. Combine them together to get the desired tail bound.
% \end{proof}

For two independent random Gaussian vectors, their inner product can be controlled with the following tail bound.
\begin{theorem}[\citealp{gao2020model}]\label{thm:inner-product-tail}
    Let $X,Y\in\Rp$ be independent random Gaussian vectors where $X_r\sim\calN(0,1)$ and $Y_r\sim\calN(0,1)$ for all $r\in[p]$, then it holds
    \begin{align*}
        \prob(|X\transpose Y| \geq \sqrt{2pt} + 2t) \leq 2e^t.
    \end{align*}
\end{theorem}

% From Theorem \ref{thm:bernstein}, we can establish a tail bound for random Gaussian vectors $b$ and $\beta(0)$.
\begin{lemma}\label{lem:inner-product-tail}
    Let $b,\beta(0)\in\Rp$ be independent random Gaussian vectors with $b_r\sim\calN(0,1)$ and $(\beta(0))_r\sim\calN(0,1)$ independently for all $r\in[p]$, then for any $p \geq 2\log\frac{2}{\delta}$ it holds with probability at least $1-\delta$ that
    \begin{align*}
        \frac{|\inner{b}{\beta(0)}|}{\sqrt{p}} \leq \sqrt{8\log\frac{2}{\delta}}.
    \end{align*}
\end{lemma}

\begin{corollary}\label{cor:W0-b-tail}
    Let $W(0)\in\Rpd$ and $b\in\Rp$ be independent random Gaussian matrix and vector with $(W(0))_{rj}\sim\calN(0,1)$ and $b_r\sim\calN(0,1)$ independently for all $r\in[p]$ and $j\in[d]$, then for any $p \geq 2\log\frac{2d}{\delta}$ it holds with probability at least $1-\delta$ that
    \begin{align*}
        \frac{\|W(0)\transpose b\|}{\sqrt{p}} \leq \sqrt{8d\log\frac{2d}{\delta}}.
    \end{align*}
\end{corollary}

\begin{corollary}\label{cor:theta-tail}
    Let $\theta(0) = X\transpose e_0 = \frac{1}{\sqrt{p}}X\transpose X W(0)\transpose\beta(0) - X\transpose y$ and $\theta_* = X\transpose y$, where $W(0)\in\Rpd$ and $\beta(0)\in\Rp$ be independent random Gaussian matrix and vector with $(W(0))_{rj}\sim\calN(0,1)$ and $(\beta(0))_r\sim\calN(0,1)$ independently for all $r\in[p]$ and $j\in[d]$ and $|y_i|\leq 1$ for all $i\in[n]$. If if $\eps \leq C$, $n \geq \frac{1}{\eps\gamma} (d\log\frac{C}{\eps} + \log\frac{1}{\delta})$, and $p \geq 2\log\frac{2d}{\delta}$, then with probability at least $1-3\delta$ that
    \begin{align*}
        \|\theta(0)\|\leq (1+\eps)\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\frac{n}{\sqrt{d}}, \qquad \|\theta_*\|\leq (1+\eps)\frac{n}{\sqrt{d}}.
    \end{align*}
\end{corollary}

\begin{proof}
    Recall that from \cref{cor:RIP} we have $\|X\|\leq (1+\eps)\sqrt{\frac{n}{d}}$ with probability at least $1-\delta$. If $|y_i|\leq 1$ for all $i\in[n]$, it holds that $\|y\|\leq \sqrt{n}$. Consequently, we have $\|\theta_*\| \leq \|X\|\|y\| \leq (1+\eps)\frac{n}{\sqrt{d}}$ with probability at least $1-\delta$. In particular, if $\eps \leq C$ and $n \geq \frac{1}{\eps\gamma} (d\log\frac{C}{\eps} + \log\frac{1}{\delta})$, it holds with probability at least $1-3\delta$ that
    \begin{align*}
        \|\theta(0)\| & \leq \frac{1}{\sqrt{p}}\|X\transpose X\|\|W(0) \beta(0)\| + \|\theta_*\| \\
        & \leq (1+\eps)\left(1 + \sqrt{8\log\frac{2d}{\delta}}\right)\frac{n}{\sqrt{d}},
    \end{align*}
    where the first inequality is due to Cauchy-Schwarz and triangular inequality, and the second inequality is due to Corollary \ref{cor:RIP,cor:W0-b-tail}.
\end{proof}

